Approximation Bounds for Sparse Programs

We show that sparsity constrained optimization problems over low dimensional spaces tend to have a small duality gap. We use the Shapley-Folkman theorem to derive both data-driven bounds on the duality gap, and an efficient primalization procedure to recover feasible points satisfying these bounds. These error bounds are proportional to the rate of growth of the objective with the target cardinality, which means in particular that the relaxation is nearly tight as soon as the target cardinality is large enough so that only uninformative features are added.

==> app_transfer.tex <==
%!TEX root = main.tex
\begin{center}{\LARGE \bf Appendices}\end{center}\vskip12pt

\textbf{Notation:}
Here we introduce several additional pieces of notation we will use throughout. 

We use $\mE_{\x}[\cdot]$ to refer to the expectation operator taken over the randomness in the vector $\x$ samples from a distribution $\Pr_{\x}$. Throughout we will use $\cF$ to refer exclusively to a scalar-valued function class of tasks and $\cH$ to a vector-valued function class of features. For $\cF$, we use $\cF^{\otimes t}$ to refer its $t$-fold Cartesian product such that $(f_1, \hdots, f_t) \equiv \f \in \cF^{\otimes t}$ for $f_j \in \cF$, $j \in [t]$. We use $f(\h)$ as shorthand for the function composition, $f \circ \h$. Similarly, we define the composed function class $\cF(\cH) = \{ f(\h) : \f \in \cF^{\otimes t}, \h \in \cH \}$ and its vector-valued version $\cF^{\otimes t}(\cH) = \{ (f_1(\h), \hdots, f_t(\h)) : f_j \in \cF$, $j \in [t], \h \in \cH \}$ with this shorthand. We will use $\gtrsim$, $\lesssim$, and $\asymp$ to denote greater than, less than, and equal to up to a universal constant and use $\tlO$ to denote an expression that hides polylogarithmic factors in all problem parameters. 

In the context of the two-stage ERM procedure introduced in \cref{sec:prelim} we let the design matrix and responses $y_{ji}$ for the $j$th task be $\X_j$ and $\y_j$ for $j \in [t] \cup \{0\}$, and the entire design matrix and responses concatenated over all $j \in [t]$ tasks as $\X$ and $\y$ respectively. Given a design matrix $\bX = (\x_1, \hdots, \x_N)^\top$ (comprised of mean-zero random vectors) we will let $\mSigma_{\bX} = \frac{1}{N} \bX^\top \bX$ denote its corresponding empirical covariance.

Recall we define the  notions of the empirical and population Gaussian complexity for a generic vector-valued function class $\cQ$ containing functions $\q(\cdot) : \mR^d \to \mR^r$, and data matrix $\X$ with $N$ datapoints as,
\begin{equation*}
\EMPGaus{\X}{\cQ} = \mE_{\g}[\sup_{\q \in \cQ} \frac{1}{N} \sum_{k=1}^r \sum_{i=1}^N g_{ki} q_k(\x_{i})], \qquad \POPGaus{N}{\cQ} = \mE_{\X} [\EMPGaus{\X}{\cQ}]  \qquad  g_{ki} \sim \cN(0, 1) \ i.i.d.,
\end{equation*}
where for the latter population Gaussian complexity each its $N$ datapoints are drawn from the $\Pr_{\x}(\cdot)$ design distribution. Analogously to the above we can define the empirical and population Rademacher complexities for generic vector-valued functions as,
\begin{equation*}
\EMPRad{\X}{\cQ} = \mE_{\bepsilon}[\sup_{\q \in \cQ} \frac{1}{N} \sum_{k=1}^r \sum_{i=1}^N \epsilon_{ki} q_k(\x_{i})], \qquad \POPRad{N}{\cQ} = \mE_{\X} [\EMPRad{\X}{\cQ}]  \qquad  \epsilon_{ki} \sim \text{Rad}(\frac{1}{2}) \ i.i.d.,
\end{equation*}



\section{Proofs in \cref{sec:transfer}}
\label{app:transfer}
We include the proofs of central generalization guarantees and the Gaussian process chain rule used in its proof.
\subsection{Training Phase/Test Phase Proofs}
\label{app:metatrainmetatest}

In all the following definitions $(\x, y)$ refer to datapoint drawn from the model in \cref{eq:gen_model}. We first include the proof of \cref{thm:metatrain} which shows that minimizing the training phase ERM objective controls the task-average distance between the underlying feature representation $\h$ and learned feature representation $\hh$.
\begin{proof}[Proof of \cref{thm:metatrain}]

For fixed $\f', \h'$, define the centered training risk as, 
\begin{align*}
	L(\f', \h', \fstar, \hstar) = \frac{1}{t}\sum_{j=1}^t  \mE_{\x, y} \Big \{ \ell(f_j' \circ \h'(\x), y) - \ell(f_j^{\star} \circ \hstar(\x), y) \Big \}.
\end{align*}
and its empirical counterpart,
\begin{align*}
	\hat{L}(\f', \h', \fstar, \hstar) = \frac{1}{t}\sum_{j=1}^t \sum_{i=1}^{n} \Big \{ \ell(f_j' \circ \h'(\x_{ji}), y_{ji}) - \mE_{\x, y}[\ell(f_j^{\star} \circ \hstar(\x), y)] \Big \}
\end{align*}

Now if $\tbf$ denotes the minimizer of the former expression for fixed $\hh$, in the sense that $\tbf = \frac{1}{t}\sum_{j=1}^t \arg \inf_{f'_j \in \cF} \mE_{\x, y} \Big \{ \ell(f'_j \circ \hh(\x), y) - \ell(f_j^{\star} \circ \hstar(\x), y) \Big \}
$, then by definition, we have that $\avdist{\fstar}{\hh}{\hstar}$ equals the former expression. We first decompose the average distance using the pair $(\hbf, \hh)$ --
\begin{align*}
L(\tbf, \hh, \fstar, \hstar) - L(\fstar, \hstar, \fstar, \hstar) = \underbrace{L(\tbf, \hh, \fstar, \hstar) - L(\hbf, \hh, \fstar, \hstar)}_{a} + L(\hbf, \hh, \fstar, \hstar) - L(\fstar, \hstar, \fstar, \hstar)
\end{align*}
Note that by definition of the $\tbf$, $a \leq 0$. The second pair can be controlled via the canonical risk decomposition, 
\begin{align*}
& L(\hbf, \hh, \fstar, \hstar) - L(\fstar, \hstar, \fstar, \hstar)
= \underbrace{L(\hbf, \hh, \fstar, \hstar) - \hat{L}(\hbf, \hh, \fstar, \hstar)}_{b} + \underbrace{ \hat{L}(\hbf, \hh, \fstar, \hstar) - \hat{L}(\fstar, \hstar, \fstar, \hstar)}_{c} + \\
& \underbrace{\hat{L}(\fstar, \hstar, \fstar, \hstar) - L(\fstar, \hstar, \fstar, \hstar)}_{d}.
\end{align*}
By definition $c \leq 0$ (note this inequality uses the realizability in \cref{assump:realizable}) and $b,d \leq \sup_{f_j \in \cF, \h \in \cH}\abs{\Ltrain(\f, \h)-\hLtrain(\f, \h)}$. By an application of the bounded differences inequality and a standard symmetrization argument (see for example \citet[Theorem 4.10]{wainwright2019high} we have that, 
\begin{align*}
	\sup_{f_j \in \cF, \h \in \cH}\abs{\Ltrain(\f, \h)-\hLtrain(\f, \h)} \leq 2 \POPRad{nt}{\ell(\cF^{\otimes t}(\cH))}] + 2 B \sqrt{\frac{\log(1/\delta)}{nt}}
\end{align*}
with probability at least $1-2\delta$.

It remains to decompose the leading Rademacher complexity term. First we center the functions to $\ell_{ji}(f_j \circ \h(\x_{ji}), y_{ji}) = \ell(f_j \circ \h(\x_{ji}), y_{ji}) - \ell(0, y_{ji})$. Then noting $\abs{\ell_{ji}(0, y_{ji})} \leq B$, the constant-shift property of Rademacher averages \citet[Exercise 4.7c]{wainwright2019high} gives, 
\begin{align*}
	\mE_{\bepsilon}[\sup_{f_j \in \cF, \h \in \cH} \frac{1}{nt} \sum_{j=1}^t \sum_{i=1}^n \epsilon_{ij} \ell(f_j \circ \h(\x_{ji}), y_{ji})] \leq \mE_{\bepsilon}[\sup_{f_j \in \cF, \h \in \cH} \frac{1}{nt} \sum_{j=1}^t \sum_{i=1}^n \epsilon_{ij} \ell_{ij}(f_j \circ \h(\x_{ji}), y_{ji})] + \frac{B}{\sqrt{nt}}
\end{align*}
Now note each $\ell_{ij}(\cdot, \cdot)$ is $L$-Lipschitz in its first coordinate uniformly for every choice of the second coordinate. So, defining the set $S=\{ f_j \circ \h(\x_{ji}) : f_j \in \cF, \h \in \cH \} \subseteq \mR^{tn}$, and applying the contraction principle \citet[Theorem 4.12]{ledoux2013probability} over this set shows,
\begin{align*}
	\mE_{\bepsilon}[\sup_{f_j \in \cF, \h \in \cH} \frac{1}{nt} \sum_{j=1}^t \sum_{i=1}^n \epsilon_{ij} \ell_{ij}(f_j \circ \h(\x_{ji}), y_{ji})] \leq 2L \cdot \POPRad{nt}{\cF^{\otimes t}(\cH)}.
\end{align*}
Combining gives,
\begin{align*}
	\sup_{f_j \in \cF, \h \in \cH}\abs{\Ltrain(\f, \h)-\hLtrain(\f, \h)} \leq 4L \cdot \POPRad{nt}{\cF^{\otimes t}(\cH)} + \frac{4B \sqrt{\log(1/\delta)}}{\sqrt{nt}}
\end{align*}

with probability $1-2\delta$. By \cite[p.97]{ledoux2013probability}, $\EMPRad{\X}{\cF^{\otimes t}(\cH)} \leq \sqrt{\frac{\pi}{2}} \EMPGaus{\X}{\cF^{\otimes t}(\cH)}$, which after taking expectations yields the first inequality in the theorem statement.

The last remaining step hinges on \cref{thm:chain_rule} to decompose the Gaussian complexity over $\cF$ and $\cH$. A direct application of \cref{thm:chain_rule} gives the conclusion that,
\begin{align*}
	\EMPGaus{\X}{\cF^{\otimes t}(\cH)} \leq 128 \left (\frac{D_{\X}}{(nt)^2} + C(\cF^{\otimes t}(\cH)) \cdot \log(nt) \right)
\end{align*}
	where $C(\cF^{\otimes t}(\cH); \X) =  L(\cF) \cdot \EMPGaus{\X}{\cH} + \max_{\Z \in \cZ} \EMPGaus{\Z}{\cF}$ where $\cZ = \{ \h(\bX) : \h \in \cH, \bX \in \cup_{j=1}^{t} \{\X_j\} \}$. By definition of $D_{\X}$ we have $D_{\X} \leq 2 D_{\cX}$ and similarly that $\max_{\Z \in \cZ} \EMPGaus{\Z}{\cF} \leq \max_{\Z \in \cZ_1} \EMPGaus{\Z}{\cF}$ for $\cZ_1 = \{ (\h(\x_1), \cdots, \h(\x_n)) ~|~ \h \in \cH, \x_i \in \cX \text{~for all~} i\in[n]\}$. Taking expectations over $\X$ in this relations and assembling the previous bounds gives the conclusion after rescaling $\delta$.
\end{proof}

An analogous statement holds both in terms of a sharper notion of the worst-case Gaussian complexity and in terms of empirical Gaussian complexities.

\begin{corollary}
	In the setting of \cref{thm:metatrain},
	\begin{align*}
     \avdist{\fstar}{\hh}{\hstar}		\leq  4096 L \left[ 
	\frac{D_{\cX}}{(nt)^2} + \log(nt) \cdot [L(\cF) \cdot \POPGaus{\X}{\cH} + \mE_{\X}[\max_{\Z \in \cZ} \EMPGaus{\Y}{\cF}]\right] + 8 B \sqrt{\frac{\log(1/\delta)}{n}}
	\end{align*}
	with probability $1-2\delta$ for $\cZ = \{ \h(\bX) : \h \in \cH, \bX \in \cup_{j=1}^{t} \{\X_j\} \}$. Furthermore, 
	\begin{align*}
		& \avdist{\fstar}{\hh}{\hstar}	 \leq 16 \EMPGaus{\X}{\cF^{\otimes t}(\cH)} + 16 B \sqrt{\frac{\log(1/\delta)}{n}}	\leq \\
		& 4096 L \left[ 	\frac{D_{\cX}}{(nt)^2} + \log(nt) \cdot [L(\cF) \cdot \EMPGaus{\X}{\cH} + \max_{\Z \in \cZ} \EMPGaus{\Z}{\cF}]\right] + 16 B \sqrt{\frac{\log(1/\delta)}{n}}	
	\end{align*}
	with probability at least $1-4\delta$. 
	\label{cor:metatrain_emp}
\end{corollary}

\begin{proof}
The argument follows analogously to the proof of \cref{thm:metatrain}. The first statement follows identically by simply avoiding the relaxation using \cref{thm:chain_rule}, $\max_{\Z \in \cZ} \EMPGaus{\Z}{\cF} \leq \max_{\Z \in \cZ_1} \EMPGaus{\Z}{\cF}$ for $\cZ_1 = \{ (\h(\x_1), \cdots, \h(\x_n)) ~|~ \h \in \cH, \x_i \in \cX \text{~for all~} i\in[n]\}.$

The second statement follows by a direct modification of  \cref{thm:metatrain}. In the proof  another application of the bounded differences inequality would show that $\abs{\POPRad{nt}{\cF^{\otimes t}(\cH)}-\EMPRad{\X}{(\cF^{\otimes t}(\cH)}} \leq 4B \sqrt{\frac{\log(1/\delta)}{nt}}$ with probability $1-2\delta$. Hence a union bound over this event and the event in the theorem, followed the steps in \cref{thm:metatrain} gives the result after a an application of \cref{thm:chain_rule}.
\end{proof}


We now show how the definition of task diversity in \cref{def:diversity} and minimizing the training phase ERM objective allows us to transfer a fixed feature representation $\hh$ and generalize to a new task-specific mapping $f_{0}$.

\begin{proof}[Proof of \cref{thm:metatest}]
Note $\tf_{0} = \argmin_{f \in \cF} \Ltest(f, \hh)$, that is the minimizer of the population test risk loaded with the fixed feature representation $\hh$. The approach to controlling this term uses the canonical risk decomposition,
\begin{align*}
\Ltest(\hf_{0}, \hh) - \Ltest(\tf_{0}, \hh)
=\underbrace{\Ltest(\hf_{0}, \hh) - \hLtest(\hf_{0}, \hh)}_{a} + \underbrace{\hLtest(\hf_{0}, \hh) - \hLtest(\tf_{0}, \hh)}_{b} + \underbrace{\hLtest(\tf_{0}, \hh) - \Ltest(\tf_{0}, \hh)}_{c}
\end{align*}
First by definition, $b \le 0$.
Now a standard uniform convergence/symmetrization argument which also follows the same steps as in the proof of \cref{thm:metatrain},
\begin{align*}
	a+c \leq 16L \cdot  \mE_{\X_0}[\EMPGaus{\Z_{\hh}}{\cF}] + 8 B \sqrt{\frac{\log(1/\delta)}{m}} \leq 16L \max_{\hh \in \cH} \mE_{\X_0}[\EMPGaus{\Z_{\hh}}{\cF}] + 8B \sqrt{\frac{\log(1/\delta)}{m}}
\end{align*}
for  $\Z_{\hh} = \hh(\X_{0})$, with probability at least $1-2\delta$. The second inequality simply uses the fact that the map $\hh$ is fixed, and independent of the randomness in the test data.
The bias from using an imperfect feature representation $\hh$ in lieu of $\h$ arises in $\Ltest(\tf_{0}, \hh)$. For this term,
\begin{align*}
	& \Ltest(\tf_{0}, \hh) - \Ltest(f_{0}, \hstar) = \inf_{\tf_{0} \in \cF} \{ \Ltest(\tf_{0}, \hh) - \Ltest(f_{0}, \hstar) \} \leq \sup_{f \in \cF_0} \inf_{\tf_{0} \in \cF} \{ L(\tf_{0}, \hh) - L(f_{0}, \hstar) \} = \\
	& \dist{\h}{\hh}
\end{align*}

To obtain the final theorem statement we use an additional relaxation on the Gaussian complexity term for ease of presentation,
\begin{align*}
    \max_{\hh \in \cH} \mE_{\X_0}[\EMPGaus{\Z_{\hh}}{\cF}] \leq \MAXGaus{m}{\cF}.
\end{align*}
Combining terms gives the conclusion. 
\end{proof}

We also present a version of \cref{thm:metatest} which can possess better dependence on the boundedness parameter in the noise terms and has better dependence on the Gaussian complexities. As before our guarantees can be stated both in terms of population or empirical quantities.
The result appeals to the functional Bernstein inequality instead of the bounded differences inequality in the concentration step. Although we only state (and use) this guarantee for the test phase generalization an analogous statement can be shown to hold for \cref{thm:metatrain}.

\begin{corollary}	
	In the setting of \cref{thm:metatest}, assuming the loss function $\ell$ satisfies the centering $\ell(0, y)=0$ for all $y \in \cY$,
\begin{align*}
\Ltest(\hf_{0}, \hh) - \Ltest(f^\star_{0}, \h^\star) \leq \dist{\hh}{\h^\star} + 16 L \cdot \mE_{\X_0}[\EMPGaus{\Z_{\hh}}{\cF}] + 4 \sigma \sqrt{\frac{\log(2/\delta)}{m}} + 50 B \frac{\log(2/\delta)}{m}
\end{align*}
for $\Z_{\hh} = \hh(\X_0)$, with probability at least $1-\delta$. Here the maximal variance $\sigma^2 = \frac{1}{m} \sup_{f \in \cF} \sum_{i=1}^m \Var(\ell(f \circ \hh(\x_i), y_i))$. Similarly we have that, 
\begin{align*}
\Ltest(\hf_{0}, \hh) - \Ltest(f^\star_{0}, \h^\star) \leq \dist{\hh}{\h^\star} + 32L \cdot  \EMPGaus{\Z_{\hh}}{\cF} + 8 \sigma \sqrt{\frac{\log(2/\delta)}{m}} + 100 B \frac{\log(2/\delta)}{m}
\end{align*}
with probability at least $1-2\delta$.
	\label{cor:metatest_funcbernstein}	
\end{corollary}
\begin{proof}[Proof of \cref{cor:metatest_funcbernstein}]
	The proof is identical to the proof of \cref{thm:metatest} save in how the concentration argument is performed. Namely in the notation of \cref{thm:metatest}, we upper bound,
	\begin{align*}
		a+c \leq 2 \sup_{f \in \cF} \abs{\hLtest(f, \hh)-\Ltest(f, \hh)} = 2 Z
	\end{align*}
	Note by definition $\mE_{\X_0, \y_0}[\hLtest(f, \hh)] = \Ltest(f, \hh)$, where $\hLtest(f, \hh) = \frac{1}{m} \sum_{i=1}^m \ell(f \circ \hh(\x_i), y_i)$, and the expectation is taken over the test-phase data. Instead of applying the bounded differences inequality to control the fluctuations of this term we apply a powerful form of the functional Bernstein inequality due to \citet{massart2000constants}. Applying \citet[Theorem 3]{massart2000constants} therein, we can conclude,
	\begin{align*}
		Z \leq (1+\epsilon) \mE[Z] + \frac{\sigma}{\sqrt{n}} \sqrt{2 \kappa \log(\frac{1}{\delta})} + \kappa(\epsilon) \frac{B}{m} \log(\frac{1}{\delta})
	\end{align*}
	for $\kappa=2$, $\kappa(\epsilon) = 2.5 + \frac{32}{\epsilon}$ and $\sigma^2 = \frac{1}{m} \sup_{f \in \cF} \sum_{i=1}^m \Var(\ell(f \circ \hh(\x_i), y_i))$. We simply take $\epsilon=1$ for our purposes, which gives the bound,
	\begin{align*}
		Z \leq 2 \mE[Z] + 4 \frac{\sigma}{\sqrt{m}} \sqrt{\log(\frac{1}{\delta})} + 35 \frac{B}{m} \log(\frac{1}{\delta})
	\end{align*}
	
	Next note a standard symmetrization argument shows that $\mE[Z] \leq 2  \mE_{\X_0, \y_0}[\EMPRad{\Z_{\hh}}{\ell \circ \cF}]$ for  $\Z_{\hh} = \hh(\X_{0})$. Following the proof of \cref{thm:metatest} but eschewing the unnecessary centering step in the application of the contraction principle shows that, $\EMPRad{\Z_{\hh}}{\ell \circ \cF} \leq 2 \EMPRad{\Z_{\hh}}{\cF}$. Upper bounding empirical Rademacher complexity by Gaussian complexity and following the steps of \cref{thm:metatest} gives the first statement.
	
	
	This population Rademacher complexity can be converted into an empirical Rademacher complexity once again using a similar concentration inequality based result which appears in a convenient form in \citet[Lemma A.4 (i)]{bartlett2005local}.  Directly applying this result (with $\alpha=\frac{1}{2}$) shows that, 
	\begin{align*}
		\mE_{\X_0, \y_0}[\EMPRad{\Z_{\hh}}{\ell \circ \cF}] \leq 2 \EMPRad{\Z_{\hh}}{\ell \circ \cF} + \frac{8B \log(\frac{1}{\delta})}{m}
	\end{align*}
	with probability at least $1-\delta$. The remainder of the argument follows exactly as in the proof of \cref{thm:metatest} along with another union bound.
\end{proof}




The proof of \cref{cor:ltlguarantee} is almost immediate.
\begin{proof}[Proof of \cref{cor:ltlguarantee}]
	The result follows immediately by combining \cref{thm:metatrain}, \cref{thm:metatest}, and the definition of task diversity along with a union bound over the two events on which \cref{thm:metatrain,thm:metatest} hold.
\end{proof}

\subsection{A User-Friendly Chain Rule for Gaussian Complexity}
\label{app:chainrule}
We provide the formal statement and the proof of the chain rule for Gaussian complexity that is used in the main text to decouple the complexity of learning the class $\cF^{\otimes t}(\cH)$ into the complexity of learning each individual class. We believe this result may be a technical tool that is of more general interest for a variety of learning problems where compositions of function classes naturally arise.  

Intuitively, the chain rule (\cref{thm:chain_rule}) can be viewed as a generalization of the Ledoux-Talagrand contraction principle which shows that for a \textit{fixed}, centered $L$-Lipschitz function $\phi$, $\EMPGaus{\X}{\phi(\cF)} \le 2 L \EMPGaus{\X}{\cF}$. However, as we are learning \textit{both} $\f \in \cF^{\otimes t}$ (which is not fixed) and $\h \in \cH$, $\EMPGaus{\X}{\cF^{\otimes t} \circ\cH }$ features a suprema over both $\cF^{\otimes t}$ and $\cH$. 

A comparable result for Gaussian processes to our \cref{thm:chain_rule} is used in \cite{maurer2016benefit} for multi-task learning applications, drawing on the chain rule of \citet{maurer2016chain}. Although their result is tighter with respect to logarithmic factors, it cannot be written purely in terms of Gaussian complexities. Rather, it includes a worst-case ``Gaussian-like" average (\citet[Eq. 4]{maurer2016benefit}) in lieu of $\EMPGaus{\cZ}{\cF}$ in \cref{thm:chain_rule}. In general, it is not clear how to sharply bound this term beyond the linear regression example considering therein. The terms appearing in \cref{thm:chain_rule} can be sharply bounded, in a direct and modular fashion, using the wealth of existing results and tools in the learning theory literature.


Our proof technique and that of \citet{maurer2016chain} both hinge on several properties of Gaussian processes. \citet{maurer2016chain} uses a powerful generalization of the Talagrand majorizing measure theorem to obtain their chain rule. We take a different path. First we use the entropy integral to pass to the space of covering numbers--where  the metric properties of the distance are used to decouple the features and tasks. Finally an appeal to Gaussian process lower bounds are used to come back to expression that involves only Gaussian complexities.

 We will use the machinery of empirical process theory throughout this section so we introduce several useful definitions we will need. We define the empirical $\ell_2$-norm as, $d_{2, \X}^2(\f(\h), \f'(\h')) = \frac{1}{t \cdot n} \sum_{j=1}^t \sum_{i=1}^{n} (f_j(\h(\x_{ji}))-f'_j(\h'(\x_{ji}))^2$, and the corresponding $u$-covering number as $N_{2, \X}(u; d_{2, \X}, \cF^{\otimes t}(\cH))$. Further, we can define the \textit{worst-case} $\ell_2$-covering number as $N_{2}(u; \cF^{\otimes t}(\cH)) = \max_{\X} N_{2, \X}(u; d_{2, \X}, \cF^{\otimes t}(\cH))$. For a vector-valued function class we define the empirical $\ell_2$-norm similarly as $d_{2, \X}^2 (\h, \h') = \frac{1}{t \cdot n} \sum_{j=1}^t \sum_{i=1}^{n} \sum_{k=1}^r (\h_k(\x_{ji})-\h_k'(\x_{ji}))^2$.

Our goal is to bound the empirical Gaussian complexity of the set $S = \{ f_j(\h(\x_{ji})) : f_j \in \cF, \h \in \cH \} \subseteq \mathbb{R}^{tn}$ or function class,
\begin{align*}
	\EMPGaus{nt}{S} = \EMPGaus{\X}{\cF^{\otimes t}(\cH)}= \frac{1}{n t} \mE[ \sup_{\f \in \cF^{\otimes t}, \h \in \cH} \sum_{j=1}^{t} \sum_{i=1}^{n} g_{ji} f_j(\h(\x_{ji})) ] ; \quad g_{ji} \sim \cN(0,1)
\end{align*}
in a manner that allows for easy application in several problems of interest. To be explicit, we also recall that,
\begin{align*}
	\EMPGaus{\X}{\cH} = \frac{1}{nt} \mE_{\g}[\sup_{\h \in \cH} \sum_{k=1}^r \sum_{j=1}^t \sum_{i=1}^n g_{kji} \h_k(\x_{ji})] ; \quad g_{kji} \sim \cN(0,1) 
\end{align*}

We now state the decomposition theorem for Gaussian complexity.
\begin{theorem}
	Let the function class $\cF$ consist of functions that are $\ell_2$-Lipschitz with constant $L(\cF)$, and have boundedness parameter $D_{\X}=\sup_{\f,\f',\h, \h'} d_{2, \X}(\f(\h), \f'(\h'))$. Further, define $\cZ = \{ \h(\bX) : \h \in \cH, \bX \in \cup_{j=1}^{t} \{\X_j\} \}$. Then the (empirical) Gaussian complexity of the function class $\cF^{\otimes t}(\cH)$ satisfies,
	\begin{align*}
		\EMPGaus{\X}{\cF^{\otimes t}(\cH)} \leq \inf_{D_{\X} \geq \delta > 0} \left \{ 4\delta + 64 C(\cF^{\otimes t}(\cH)) \cdot \log \left( \frac{D_{\X}}{\delta} \right) \right \} \leq \frac{4  D_{\X}}{(nt)^2} + 128 C(\cF^{\otimes t}(\cH)) \cdot \log \left( nt \right)
		% C(\cF^{\otimes t}_{\cH}) \cdot \left( 1+\log \left(\frac{D_{\X}}{C(\cF^{\otimes t}(\cH))} \right) \right)
	\end{align*}
	where $C(\cF^{\otimes t}(\cH)) =  L(\cF) \cdot \EMPGaus{\X}{\cH} + \max_{\Z \in \cZ} \EMPGaus{\Z}{\cF}$. Further, if $C(\cF^{\otimes t}(\cH)) \leq D_{\X}$ then by computing the exact infima of the expression,
	\begin{align*}
		\EMPGaus{\X}{\cF^{\otimes t}(\cH)} \leq 64 \left( C(\cF^{\otimes t}(\cH)) + C(\cF^{\otimes t}(\cH)) \cdot \log \left( \frac{D_{\X}}{C(\cF^{\otimes t}(\cH))} \right) \right)
	\end{align*}
	\label{thm:chain_rule}
\end{theorem}

\begin{proof}
For ease of notation we define $N=nt$ in the following.
We can rewrite the Gaussian complexity of the function class $\cF^{\otimes t}(\cH)$ as,
\begin{align*}
	 \EMPGaus{\X}{\cF^{\otimes t}(\cH)} = \mE[\frac{1}{nt} \sup_{\f (\h) \in \cF^{\otimes t}(\cH)} \sum_{j=1}^{t} \sum_{i=1}^{n} g_{ji} f_j(\h(\x_{ji}))] = \mE[\frac{1}{\sqrt{N}} \cdot \sup_{\f (\h) \in \cF^{\otimes t}(\cH)} Z_{\f(\h)}]
\end{align*}
from which we define the mean-zero stochastic process $ Z_{\f(\h)} = \frac{1}{\sqrt{N}} \sum_{j=1}^t \sum_{i=1}^{n} g_{ji} f_j(\h(\x_{ji}))$ for a fixed sequence of design points $\x_{ji}$, indexed by elements $\{ \f(\h) \in \cF^{\otimes t}(\cH) \}$, for a sequence of independent Gaussian random variables $g_{ji}$. Note the process $Z_{\f(\h)}$ has sub-gaussian increments, in the sense that,
	$Z_{\f(\h)}-Z_{\f'(\h')}$ is a sub-gaussian random variable with parameter $d_{2, \X}^2(\f(\h), \f'(\h')) = \frac{1}{N} \sum_{j=1}^t \sum_{i=1}^{n} (f_j(\h(\x_{ji}))-f'_j(\h'(\x_{ji}))^2$. Since $Z_{\f(\h)}$ is a mean-zero stochastic process we have that, $\mE[\sup_{\f(\h) \in \cF^{\otimes t}(\cH)} Z_{\f(\h)} ] = \mE[\sup_{\f(\h) \in \cF^{\otimes t}(\cH)} Z_{\f(\h)} - Z_{\f'(\h')}] \leq \mE[\sup_{\f(\h), \f'(\h') \in \cF^{\otimes t}(\cH)} Z_{\f(\h)} - Z_{\f'(\h')}]$. Now an appeal to the Dudley entropy integral bound, \citet[Theorem 5.22]{wainwright2019high} shows that,
		\begin{align*} \mE[\sup_{\f(\h), \f(\h') \in \cF^{\otimes t}(\h)} Z_{\f(\h)} - Z_{\f(\h')}] \leq & 4 \mE[\sup_{d_{2, \X}(\f(\h), \f(\h')) \leq \delta} Z_{\f(\h)}-Z_{\f(\h')}] +  32 \int_{\delta}^{D} \sqrt{\log N_{\X}(u; d_{2, \X}, \cF^{\otimes t}(\cH))} du.
		\end{align*}
		We now turn to bounding each of the above terms. Parametrizing the sequence of i.i.d. gaussian variables as $\g$, it follows that $\sup_{d_{2, \X}(\f(\h), \f(\h')) \leq \delta}  Z_{\f(\h)}-Z_{\f(\h')} \leq \sup_{\v : \norm{\v}_2 \leq \delta} \g \cdot \v \leq \norm{\g} \delta$. The corresponding expectation bound, after an application of Jensen's inequality to the $\sqrt{\cdot}$ function gives $\mE[\sup_{d_{2, \X}(\f(\h), \f(\h')) \leq \delta} Z_{\f(\h)}-Z_{\f(\h')}] \leq \mE[\norm{\g}_2 \delta] \leq \sqrt{N} \delta$.
		
		We now turn to bounding the second term by decomposing the distance metric $d_{2, \X}$ into a distance over $\cF^{\otimes t}$ and a distance over $\cH$, and use a covering argument on each of the spaces $\cF^{\otimes t}$ and $\cH$ to witness a covering of the composed space $\cF^{\otimes t}(\cH)$. Recall we refer to the entire dataset concatenated over the $t$ tasks as $\X \equiv \{ \x_{ji} \}_{j=1, i=1}^{t, n}$. First, let $C_{\cH_{\X}}$ be a covering of the of function space $\cH$ in the empirical $\ell_2$-norm with respect to the inputs $\X$ at scale $\epsilon_1$. Then for each $\h \in C_{\cH_{\X}}$, construct an $\epsilon_2$-covering, $C_{\cF^{\otimes t}_{\h(\X)}}$, of the function space $\cF^{\otimes t}$ in the empirical norm with respect to the inputs $\h(\X)$ at scale $\epsilon_2$. We then claim that set $C_{\cF^{\otimes t}(\cH))} = \cup_{\h \in \cH_{\X}} ( C_{\cF^{\otimes t}_{\h(\X)}} )$ is an $\epsilon_1 \cdot L(\cF) + \epsilon_2$-cover for the function space $\cF^{\otimes t}(\cH)$ in the empirical $\ell_2$ norm over the inputs $\X$.
		To see this, let $\h \in \cH$ and $\f \in \cF^{\otimes t}$ be arbitrary. Now let $\h' \in C_{\cH_{\X}}$ be $\epsilon_1$-close to $\h$. Given this $\h'$, let $\f$ be $\epsilon_2$-close to $\f' \in C_{\cF^{\otimes t}_{\h'(\X)}}$. By construction $(\h', \f') \in C_{\cF^{\otimes t}(\cH)}$.
		Finally, using the triangle inequality, we have that,
		\begin{align*}
			& d_{2, \X}(\f(\h), \f'(\h')) \leq d_{2, \X}(\f(\h), \f(\h')) + d_{2, \X}(\f(\h'), \f'(\h')) = \\
			& \sqrt{\frac{1}{N} \sum_{j=1}^t \sum_{i=1}^{n} (f_j(\h(\x_{ji}))-f_j(\h'(\x_{ji})))^2} + 
			\sqrt{\frac{1}{N} \sum_{j=1}^t  \sum_{i=1}^{n} (f_j(\h'(\x_{ji}))-f_j'(\h'(\x_{ji})) )^2} \leq \\
			& L(\cF) \sqrt{\frac{1}{N} \sum_{k=1}^{r} \sum_{j=1}^t \sum_{i=1}^{n} (\h_k(\x_{ji})-\h_k'(\x_{ji}))^2} + 
			\sqrt{\frac{1}{N} \sum_{j=1}^t  \sum_{i=1}^{n} (f_j(\h'(\x_{ji}))-f_j'(\h'(\x_{ji})) )^2} = \\
			& L(\cF) \cdot d_{2, \X}(\h, \h') + d_{2, \h'(\X)}(\f, \f') \leq \epsilon_1 \cdot L(\cF) + \epsilon_2
		\end{align*}
	appealing to the uniform Lipschitz property of the function class $\cF$ in moving from the second to third line, which establishes the claim.
	The cardinality of $C_{\cF^{\otimes t}_{\cH}}$ can also be bounded as $\abs{C_{\cF^{\otimes t}_{\cH}}} = \sum_{\h \in C_{\cH_{\X}}} \abs{C_{\cF^{\otimes t}_{\h(\X)}}} \leq \abs{C_{\cH_{\X}}} \cdot \max_{\h \in \cH_{\X}} \abs{C_{\cF^{\otimes t}_{\h(\X)}}} $. Further, $\max_{\h \in \cH_{\X}} \abs{C_{\cF^{\otimes t}_{\h(\X)}}} \leq \abs{\underbrace{\max_{\z \in \cZ} C_{\cF_{\z}} \times \hdots \times \max_{\z \in \cZ} C_{\cF_{\z}}}_{t \text{ times}}} \leq \abs{\max_{\z \in \cZ} C_{\cF_{\z}}}^t$ -- note that an $\epsilon$-cover of $\cF^{\otimes t}_{\h(\X)}$ in the empirical $\ell_2$-norm with respect to $\h(\X)$ can be obtained from the cover $C_{\cF_{\h(\X_1)}} \times \hdots \times C_{\cF_{\h(\X_t)}}$ where $C_{\cF_{\h(\X_i)}}$ denotes a $\epsilon$-cover of $\cF$ in the empirical $\ell_2$-norm with respect to $\h(\X_i)$. Thus, it follows, that,
	\begin{align*}
		\log N_{2, \X}(\epsilon_1 \cdot L(\cF) + \epsilon_2, d_{2, \X}, \cF^{\otimes t}(\cH)) \leq \log N_{2, \X}(\epsilon_1, d_{2, \X}, \cH) + t \cdot \max_{\Z \in \cZ} \log N_{2, \Z}(\epsilon_2, d_{2, \Z}, \cF)	
	\end{align*}

Using the covering number upper bound with $\epsilon_1=\frac{\epsilon}{2\cdot L(\cF)}$, $\epsilon_2 = \frac{\epsilon}{2}$ and sub-additivity of the $\sqrt{\cdot}$ function shows,
	\begin{align*}
		\int_{\delta}^{D} \sqrt{\log N_2(\epsilon, d_{2, \X}, \cF^{\otimes t}(\cH))}	 \ d\epsilon \leq \int_{\delta}^D \sqrt{\log N_{2, \X}(\epsilon/(2 L(\cF)), d_{2, \X}, \cH)} \ d \epsilon + \sqrt{t} \int_{\delta}^{D} \max_{\Z \in \cZ} \sqrt{\log N_{2, \Z} (\frac{\epsilon}{2}, d_{2, \Z}, \cF)} \ d \epsilon
	\end{align*}
	From the Sudakov minoration theorem \citet{wainwright2019high}[Theorem 5.30] for Gaussian processes and the fact packing numbers at scale $u$ upper bounds the covering number at scale $u$ we obtain that\footnote{For the $\cH$ term  we can apply the result to the mean-zero Gaussian process $Z_{\h} = \frac{1}{\sqrt{nt}} \sum_{k=1}^r \sum_{j=1}^t \sum_{i=1}^n g_{kji} h_k(\x_{ji})$, with $g_{kji} \sim \cN(0,1)$ i.i.d., and $\h \in \cH$.}
	\begin{align*}
			\log N_{2, \X}(u; d_{2, \X}, \cH) \leq 4 \left (\frac{\sqrt{nt} \EMPGaus{\X}{\cH}}{u} \right)^2 \ \forall  u>0
			\quad \text{ and } \quad \log N_{2, \Z}(u; d_{2, \Z}, \cF) \leq 4 \left( \frac{\sqrt{n} \EMPGaus{\Z}{\cF}}{u} \right)^2 \ \forall  u>0.
	\end{align*}
	Combining all of the aforementioned upper bounds, shows that
	\begin{align*}
		& \EMPGaus{\X}{\cF^{\otimes t}(\cH)} \leq \frac{1}{\sqrt{nt}} \left( 4 \delta \sqrt{nt} + 64 L(\cF) \cdot \EMPGaus{\X}{\cH} \cdot \sqrt{nt} \int_{\delta}^{D_{\X}} \frac{1}{u} du  +  64 \sqrt{nt} \cdot \max_{\Z \in \cZ} \EMPGaus{\Z}{\cF} \int_{\delta}^{D_{\X}} \frac{1}{u} du \right) \leq \\
		& 4\delta + 64(L(\cF) \cdot \EMPGaus{\X}{\cH} + \max_{\Z \in \cZ} \EMPGaus{\Z}{\cF}) \cdot \log \left(\frac{D_{\X}}{\delta} \right)  = \delta + C(\cF^{\otimes t}(\cH)) \cdot \log \left(\frac{D_{\X}}{\delta} \right)
		\end{align*}
	defining $C(\cF^{\otimes t}(\cH)) = L(\cF) \cdot \EMPGaus{\X}{\cH} + \max_{\Z \in \cZ} \EMPGaus{\Z}{\cF}$. Choosing $\delta=D_{\X}/(nt)^2$  gives the first inequality. Balancing first and second term gives $\delta = \frac{1}{C(\cF^{\otimes t}(\cH))}$ for the second. 
\end{proof}






==> bounds.tex <==
%!TEX root = nonlin.tex
\section{Duality Gap Bounds}
\label{sec:bounds}

Now that we have the equivalent primal, dual and bidual representations, we are ready to provide explicit bounds on \eqref{eq:primal}. Our bound construction invokes the seminal result of \citep{Aubi76} (see also \citep{Ekel99, Udel16, dAsp17} for a more recent discussion) which are briefly summarized below for the sake of completeness. 


\subsection{Duality gap bounds}

\subsection{Bounds on \eqref{eq:primal}}
Using the results of Section \ref{sec:bounds}, we can provide upper and lower bounds on the duality gap for \eqref{eq:primal}.

\begin{lemma}\label{lemma:sf}
Let $p^\ast(k)$ and $d^\ast(k)$ be defined as in \eqref{eq:primal-eqcons} and \eqref{eq:dual-eqcons} respectively. Then for some $M > 0$, we have
\begin{align*}
   p^\ast(k + \bar{k}) \leq d^\ast(k) \leq p^\ast (k) \leq d^\ast(k - \bar{k})
\end{align*}
where $k \geq (r+1)$ and $\bar{k} = \lfloor M(r+1) \rfloor$.
\end{lemma}
\begin{proof}
Since the objective in \eqref{eq:primal-eqcons} is separable, we can write the problem in perturbation form as
\begin{align*}
    h_P(u) = &\min_{x,z} \; \dfrac{1}{2}x^\top \Lambda x + \dfrac{1}{2} z^\top z + p^\top x  \tag{P-QP} \\
    \text{s.t} & \hspace{5mm} L^\top x = z + u_1 \nonumber \\
     & \hspace{5mm} \sum_{i=1}^m  \ones_{x_i \not = 0} \leq k + u_2 \nonumber
\end{align*}
where $u \in \mathbb{R}^{r + 1}$ is a perturbation vector. By construction, we have $d^\ast(k) = -h_P(0)$ and $d^\ast(k + l) = -h_P((0,l))$. Note that the function $\ones_{x_i \not = 0}$ is lower semicontinuous and that all functions in question are 1-coercive, hence satisfying Assumption 1 above.\\

We can bound the lack of convexity of of $\ones_{x_i \not = 0}$ for all $i$ by a constant $M$ which is a function of the problem parameters $\Lambda, L, p$. Consequently,
\begin{align*}
    \rho(\textbf{1}_{x \not = 0}) = \sup_{\|x\|_\infty \leq M + 1} \ones_{x \not = 0} - |x| = M
\end{align*}
where we use the fact that we can artificially make the domain of the problem compact by adding a constraint of the form $\|x\|_\infty \leq M + 1$ for $M$ large enough. This means that in the statement of Theorem \ref{th:sf} that $\max_i \rho(g_{ji}) = M$ (note that the lack of convexity measure for the equality constraints are 0). Hence our perturbation vector $\bar{p} = (0, M)$ and because were are $r+1$ constraints in \eqref{eq:primal-eqcons}, we have that
\begin{align*}
    h_P(\bar{p}) = h_P((0,M(r+1))) = d^\ast(k + M(r+1))
\end{align*}
Since the objective function is convex and separable, we have that $\max_i \rho(f_i) = 0$ and hence via Theorem \ref{th:sf} we have that
\begin{align*}
    p^\ast(k + \lfloor M(r+1)\rfloor) \leq d^\ast(k)
\end{align*}
where we introduce the floor function since $\|x\|_0 \leq \eta$ is the same for all $\eta \in [n,n+1)$ for $n \in \mathbb{N}$. The other bound follows immediately from weak duality.
\end{proof}
In Section \ref{sec:expt}, we show that empirically $M$ is not too large and that for low rank factor models the gap is often tight.

\subsection{Primalization}
We now use the results of Lemma \ref{lemma:sf} to construct a solution 



==> defs.tex <==
% Colors
\definecolor{ddarkbrown}{rgb}{0.5,0.2,0.05} \definecolor{bbluegray}{rgb}{0.05,0,0.5}

\newcommand{\blue}{\color{blue}}

% Numbering (by section, then sequential)
%\newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \renewenvironment{proof}{\textbf{Proof.}}{\QED\bigskip}
% \newtheorem{assumption}[theorem]{Assumption}


% some traditional defintions that can be blamed on craig barratt
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}
\newcommand{\BBM}{\begin{bmatrix}}
\newcommand{\EBM}{\end{bmatrix}}

% arash added these two
\newcommand{\BA}{\begin{array}}
\newcommand{\EA}{\end{array}}

% Refs, etc
\newcommand{\refp}[1]{(\ref{#1})}

% text abbrevs
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}
\newcommand{\ones}{\mathbf 1}

% std math stuff
\newcommand{\reals}{{\mathbb R}}
\newcommand{\sreals}{\scriptsize{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\complex}{{\mbox{\bf C}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

% lin alg stuff
\newcommand{\Span}{\mbox{\textrm{span}}}
\newcommand{\Range}{\mbox{\textrm{range}}}
\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\diam}{\mathop{\bf diam}}
\newcommand{\sphere}{{\mathbb S}}
\newcommand{\Nullspace}{\mbox{\textrm{nullspace}}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\NumRank}{\mathop{\bf NumRank}}
\newcommand{\NumCard}{\mathop{\bf NumCard}}
\newcommand{\Card}{\mathop{\bf Card}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}
%XXX dumb question: do we not use \diag(...) to form diagonal or 
%block diagonal matrices?
\newcommand{\idm}{\mathbf{I}}

% probability stuff
\newcommand{\Expect}{\textstyle\mathop{\bf E}}
\newcommand{\Median}{\textstyle\mathop{\bf M}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\erf}{\mathop{\bf erf}}

% convexity & optimization stuff
\newcommand{\Co}{{\mathop {\bf Co}}}
\newcommand{\co}{{\mathop {\bf Co}}}
\newcommand{\Ext}{{\mathop {\bf Ext}}}
\newcommand{\Var}{\mathop{\bf var{}}}
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\Ltwo}{{\bf L}_2}
\newcommand{\QED}{~~\rule[-1pt]{6pt}{6pt}}\def\qed{\QED}
\newcommand{\approxleq}{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\epi}{\mathop{\bf epi}}
%\newcommand{\hypo}{\mathop{\bf hypo}}
\newcommand{\var}{\mathop{\bf var}}

\newcommand{\vol}{\mathop{\bf vol}}
\newcommand{\Vol}{\mathop{\bf vol}}

\newcommand{\dom}{\mathop{\bf dom}}
\newcommand{\aff}{\mathop{\bf aff}}
\newcommand{\cl}{\mathop{\bf cl}}
\newcommand{\Angle}{\mathop{\bf angle}}
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\relint}{\mathop{\bf rel int}}
\newcommand{\bd}{\mathop{\bf bd}}
\newcommand{\vect}{\mathop{\bf vec}}
\newcommand{\dsp}{\displaystyle}
\newcommand{\foequal}{\simeq}
\newcommand{\VOL}{{\mbox{\bf vol}}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\xopt}{x^{\rm opt}}

%the following ones seem way too specialized to be here...
%let's omve them to a new file called defs2.tex or something like that
\newcommand{\Xb}{{\mbox{\bf X}}}
\newcommand{\xst}{x^\star}
\newcommand{\varphist}{\varphi^\star}
\newcommand{\lambdast}{\lambda^\star}
\newcommand{\Zst}{Z^\star}
\newcommand{\fstar}{f^\star}
\newcommand{\xstar}{x^\star}
\newcommand{\xc}{x^\star}
\newcommand{\lambdac}{\lambda^\star}
\newcommand{\lambdaopt}{\lambda^{\rm opt}}

% defs for cones & generalized inequalities
\newcommand{\geqK}{\mathrel{\succeq_K}}
\newcommand{\gK}{\mathrel{\succ_K}}
\newcommand{\leqK}{\mathrel{\preceq_K}}
\newcommand{\lK}{\mathrel{\prec_K}}
\newcommand{\geqKst}{\mathrel{\succeq_{K^*}}}
\newcommand{\gKst}{\mathrel{\succ_{K^*}}}
\newcommand{\leqKst}{\mathrel{\preceq_{K^*}}}
\newcommand{\lKst}{\mathrel{\prec_{K^*}}}
\newcommand{\geqL}{\mathrel{\succeq_L}}
\newcommand{\gL}{\mathrel{\succ_L}}
\newcommand{\leqL}{\mathrel{\preceq_L}}
\newcommand{\lL}{\mathrel{\prec_L}}
\newcommand{\geqLst}{\mathrel{\succeq_{L^*}}}
\newcommand{\gLst}{\mathrel{\succ_{L^*}}}
\newcommand{\leqLst}{\mathrel{\preceq_{L^*}}}
\newcommand{\lLst}{\mathrel{\prec_{L^*}}}

% From Alex
\newcommand{\realsp}{\mathbb{R}_+^n}
\newcommand{\intrealsp}{\int_{\mathbf{R}_+^n}}




==> dual.tex <==
%!TEX root = nonlin.tex
\section{Dual}
\label{sec:dual}

\subsection{Primal Reformulation}
We introduce two reformulations of the primal problem \eqref{eq:primal} that are equivalent to each other.
\begin{lemma}
\begin{align}\label{eq:primal-eqcons}
    p^\ast(k) = &\min_{z, \|x\|_0 \leq k} \; \dfrac{1}{2}x^\top \Lambda x + \dfrac{1}{2} z^\top z + p^\top x  \tag{P-QP} \\
    \text{s.t} & \hspace{5mm} L^\top x = z \nonumber
\end{align}
and
\begin{align}\label{eq:primal-sdp}
    p^\ast(k) = &\min_{t, u \in \{0,1\}^m} \; \dfrac{1}{2}t \tag{P-SDP} \\
    \text{s.t} & \hspace{5mm} \begin{bmatrix}
    t + p^\top \Sigma_u p & p^\top \Sigma_u L  \\
    L^\top \Sigma_u p & I_k + L^\top \Sigma_u L 
    \end{bmatrix} \succeq 0 \nonumber \\
    & \hspace{5mm} \Sigma_u = \Lambda^{1/2} \diag(u) \Lambda^{1/2} \nonumber \\
    & \hspace{5mm} \ones^\top u \leq k \nonumber
\end{align}
and
\begin{align}\label{eq:primal-saddle}
    p^\ast(k) = &\min_{\substack{z \\ u \in \{0,1\}^m \\ \ones^\top u \leq k}}  \dfrac{1}{2} p^\top \Sigma_u p + \dfrac{1}{2}\|z\|_2^2 + \dfrac{1}{2}(z + L^\top \Sigma_u p)^\top (L^\top \Sigma_u L)^{-1} (z + L^\top \Sigma_u p)  \tag{P-MM}
\end{align}
\end{lemma}
\begin{proof}
The equivalence between \eqref{eq:primal} and \eqref{eq:primal-eqcons} follows immediately. To arrive at \eqref{eq:primal-sdp}, we start from \eqref{eq:primal} and make the variable substitution $x = \diag(u) v = \diag(u) v$ where $v \in \mathbb{R}^m$ and $u \in \{0,1\}^m$ with $\ones^\top u \leq k$. We then have
\begin{align}\label{eq:primal-boolean}
    p^\ast(k) = \min_{\substack{u \in \{0,1\}^m \\ \ones^\top u \leq k}} \min_v \dfrac{1}{2}v^\top \diag(u) \Big( \Lambda + LL^\top \Big) \diag(u) v + p^\top \diag(u) v
\end{align}
We first compute the inner minimization over $v$. Note that at optimum, the sparsity pattern of $v$ must follow that of $u$ since $\Lambda \succ 0$. As a result, $v^\top \diag(u) \Lambda \diag(u) v = v^\top \Lambda v$. Setting the gradient with respect to $v$ equal to 0, we find that
\begin{align*}
    v^\ast = -\Big(\Lambda + \diag(u) LL^\top \diag(u)\Big)^{-1} \diag(u)p
\end{align*}
and after substituting back into the objective and using the fact that $(\diag(u))^2 = \diag(u^2)$ and the Woodbury matrix identity
\begin{align*}
\Big(\Lambda + \diag(u) LL^\top \diag(u)\Big)^{-1} = \Lambda^{-1} - \Lambda^{-1} \diag(u) L \Big(I_r + L^\top \diag(u) L\Big)^{-1} L^\top \diag(u) \Lambda^{-1}
\end{align*}
we have that
\begin{align*}
    p^\ast(k) = \min_{\substack{u \in \{0,1\}^m \\ \ones^\top u \leq k}} \dfrac{1}{2}p^\top \Big(\Sigma_u - \Sigma_u L(I_r + L^\top \Sigma_u L)^{-1} L^\top \Sigma_u \Big) p
\end{align*}
where $\Sigma_u = \Lambda^{1/2} \diag(u) \Lambda^{1/2}$. The result follows by introducing a slack variable $t$ and using Schur complements. Note additionally that
\begin{align*}
    p^\ast(k) &= \min_{\substack{v \in \mathbb{R}^r, u \in \{0,1\}^m \\ \ones^\top u \leq k}} \dfrac{1}{2} p^\top \Sigma_u p + \dfrac{1}{2}v^\top (I_k + L^\top \Sigma_u L ) v - v^\top L^\top \Sigma_u p  \\
    &= \min_{\substack{v \in \mathbb{R}^r, u \in \{0,1\}^m \\ \ones^\top u \leq k}} \dfrac{1}{2}\sum_{i=1}^m \; u_i \Big[\lambda_i p_i^2 + (1 + \lambda_i)(\ell_i^\top v)^2 - (\lambda_i p_i) (\ell_i^\top v) \Big]\\
\end{align*}

To arrive at \eqref{eq:primal-saddle} we start with \eqref{eq:primal-boolean} and make the variable substitution $z = L^\top \diag(u) v$. After dualizing the aforementioned constraint and noticing that strong dualilty holds for the inner most saddle point problem we have
\begin{align*}
    p^\ast(k) = \min_{\substack{u \in \{0,1\}^m \\ \ones^\top u \leq k}} \max_\nu \min_{v,z} \dfrac{1}{2}v^\top \diag(u) \Lambda \diag(u) z + \dfrac{1}{2} \|z\|_2^2 + p^\top \diag(u) v + \nu^\top (L^\top \diag(u) v - z)
\end{align*}
As before, at optimum the sparsity pattern of $v$ must follow that of $u$ and as a result we can simplify the quadratic term in $v$ to $v^\top \Lambda v$. Computing the inner minimization in $v$ we arrive at
\begin{align*}
    v^\ast = - \Lambda^{-1}\diag(u) (p + L\nu)
\end{align*}
Finally plugging back in and changing the inner max and min again via strong duality, the problem reduces to
\begin{align*}
    p^\ast(k) &= \min_{\substack{z \\ u \in \{0,1\}^m \\ \ones^\top u \leq k}} \max_\nu  \dfrac{1}{2} \|z\|_2^2 - \nu^\top z - \dfrac{1}{2} (p + L\nu)^\top \diag(u) \Lambda \diag(u) (p + L\nu) \\
    &= \min_{\substack{z \\ u \in \{0,1\}^m \\ \ones^\top u \leq k}} \max_\nu  \dfrac{1}{2} \|z\|_2^2 - \nu^\top z - \dfrac{1}{2} (p + L\nu)^\top \Lambda^{1/2} \diag(u) \Lambda^{1/2} (p + L\nu)
\end{align*}
where we use the fact that $\diag(u) \Lambda \diag(u) = \Lambda^{1/2} \diag(u) \Lambda^{1/2}$.
Computing the maximization over $\nu$ completes the proof. 
\end{proof}

\subsection{Dual problem}
While both formulations are equivalent, we concern ourselves with the dual of \eqref{eq:primal-eqcons} since it is simpler to compute.

\begin{lemma}
The dual of \eqref{eq:primal-eqcons} is
\begin{align}\label{eq:dual-eqcons}
    d^\ast(k) = \max_\nu \left\{-\dfrac{1}{2} \|\nu\|_2^2 - s_k\left(\tfrac{1}{2\lambda_{i}} (p_i + \ell_i^\top \nu)^2\right)\right\} \tag{D-QP}
\end{align}
where $s_k(\cdot)$ is the sum of the top $k$ entries of a vector.
\end{lemma}

\begin{proof}
For visual clarity, we rewrite $d^\ast(k)$ as $d^\ast$ throughout the proof. Dualizing the equality constraint we have
\begin{align*}
d^\ast = \max_{\nu}  g(\nu)
\end{align*}
where
\begin{align*}
g(\nu) = \min_{z, \|x\|_0 \leq k} \;\; \dfrac{1}{2} x^\top \Lambda x + \dfrac{1}{2}\|z\|_2^2 + p^\top x + \nu^\top(L^\top x - z)
\end{align*}
The minimization over $z$ is trivial: $z^\ast = \nu$. Hence we arrive at
\begin{align*}
d^\ast = \max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 +   \min_{\|x\|_0 \leq k}  \dfrac{1}{2} x^\top \Lambda x  + x^\top (p + L\nu)
\end{align*}
Introducing an index set $\mathcal{I}$ such that $\mathcal{I} \subseteq \{1,\hdots,m\}$ and $|\mathcal{I} | \leq k$ and on $\mathcal{I}^C$ we have $x = 0$. Letting $\lambda_i = \Lambda_{ii}$ and letting $\ell_i^\top$ denote the $i$th row of $L$, we have that
\begin{align*}
d^\ast &= \max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 +   \min_{\mathcal{I} \subseteq \{1,\hdots,n\}, |\mathcal{I}| \leq k} \min_x \;  \sum_{i \in \mathcal{I}} \; \dfrac{1}{2}\lambda_i x_i^2  + x_i (p_i + \ell_i^\top \nu) + \sum_{i \in \mathcal{I}^C} 0 \\
&= \max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 +   \min_{\mathcal{I} \subseteq \{1,\hdots,n\}, |\mathcal{I}| \leq k} \;  \sum_{i \in \mathcal{I}} \; \min_{x_i} \dfrac{1}{2}\lambda_i x_i^2  + x_i (p_i + \ell_i^\top \nu) + \sum_{i \in \mathcal{I}^C} 0 
\end{align*}
Solving the inner minimization over $x_i$ we have that
\begin{align*}
d^\ast &= \max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 +   \min_{\mathcal{I} \subseteq \{1,\hdots,n\}, |\mathcal{I}| \leq k} \;  \sum_{i \in \mathcal{I}}  -\dfrac{1}{2\lambda_i} (p_i + \ell_i^\top \nu)^2 + \sum_{i \in \mathcal{I}^C} 0 
\end{align*}
We can rewrite the optimization over $\mathcal{I}$ equivalently as 
\begin{align*}
\min_{\mathcal{I} \subseteq \{1,\hdots,n\}, |\mathcal{I}| \leq k} \;  \sum_{i \in \mathcal{I}}  -\dfrac{1}{2\lambda_i} (p_i + \ell_i^\top \nu)^2 + \sum_{i \in \mathcal{I}^C} 0  = \min_{u \in \{0,1\}^n, \; \textbf{1}^\top u \leq k} \; u^\top \alpha + (1-u)^\top 0
\end{align*}
where $\alpha_i = -\tfrac{1}{2\lambda_i} (p_i + \ell_i^\top \nu)^2$. Hence we have
\begin{align*}
-d^\ast &= -\max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 + \min_{u \in \{0,1\}^n, \; \textbf{1}^\top u \leq k} \; u^\top \alpha  \\
&= \min_{\nu} \dfrac{1}{2} \|\nu\|_2^2 - \max_{u \in \{0,1\}^n, \; \textbf{1}^\top u \leq k} \; -u^\top \alpha
\end{align*}
Note the inner minimization reduces to the sum of the top $k$ entries of $-\alpha$ and hence the problem writes
\begin{align*}
-d^\ast = -\min_\nu \dfrac{1}{2} \|\nu\|_2^2 + s_k(-\alpha)
\end{align*}
where $s_k( \cdot)$ denotes the sum of the top $k$ entries of a vector. The dual problem is (as expected) convex.
\end{proof}

\subsection{Bidual problem}
We now compute the bidual of \eqref{eq:dual-eqcons} and show that it is equivalent to the interval relaxation of \eqref{eq:primal-sdp}.
\begin{lemma}
A dual of \eqref{eq:dual-eqcons} (i.e. a bidual of \eqref{eq:primal-eqcons}) is equivalent to the interval relaxation of \eqref{eq:primal-sdp}, namely
\begin{align}\label{eq:BD-QP}
    p^{\ast \ast}(k) = &\min_{u \in [0,1]^m} \; \dfrac{1}{2}t \tag{BD-QP} \\
    \text{s.t} & \hspace{5mm} \begin{bmatrix}
    t + p^\top \Sigma_x p & p^\top \Sigma_x L  \\
    L^\top \Sigma_x p & I_k + L^\top \Sigma_x L 
    \end{bmatrix} \succeq 0 \nonumber \\
    & \hspace{5mm} \Sigma_x = \Lambda^{1/2} \diag(u) \Lambda^{1/2} \nonumber \\
    & \hspace{5mm} \ones^\top u \leq k \nonumber
\end{align}
\end{lemma}
\begin{proof}
For visual clarity, we write $d^\ast(k)$ as $d^\ast$ and $p^{\ast \ast}(k)$ as $p^{\ast \ast}$ throughout the proof. Note that
\begin{align*}
s_k(c) = \min_{\lambda \geq 0} \; \lambda k + \sum_{i=1}^n \max(0, c_i - \lambda)
\end{align*}
and the dual of $s_k(\cdot)$ can be written as 
\begin{align*}
\max_{x \in [0,1]^m} x^\top c \;\; : \;\; \textbf{1}^\top x \leq k 
\end{align*}
where we introduce a slack variable for the $\max(0,c_i - \lambda)$ term, dualize using two dual variables, and then eliminate one of the dual variables.
Using this we have that
\begin{align*}
-p^{\ast\ast} = -d^\ast = \min_\nu \max_{u \in \mathcal{C}_k} \dfrac{1}{2} \|\nu\|_2^2 - u^\top \alpha 
\end{align*}
where $\mathcal{C}_k = \{ u \; | \; \textbf{1}^\top x \leq k, \; x \in [0,1]^m \}$. By Sion's minimiax theorm, we can exchange the min and max to arrive at
\begin{align*}
-p^{\ast \ast} = \max_{u \in \mathcal{C}_k} \min_\nu  \dfrac{1}{2} \|\nu\|_2^2 - u^\top \alpha 
\end{align*}
Note that $u^\top \alpha = -\dfrac{1}{2}(p + L\nu)^\top \Lambda^{-1/2} \diag(u) \Lambda ^{-1/2} (p+L\nu)$ where $\diag(u) = \diag(u_1,\hdots,u_m)$ . Taking the minimization over $\nu$ we have
\begin{align*}
\nu^\ast = (I + L^\top D^{-1/2} \diag(u) D^{-1/2} L)^{-1} L^\top D^{-1/2} \diag(u) D^{-1/2} p
\end{align*}
Plugging back in, our objective reduces to
\begin{align*}
-p^{\ast \ast} = \max_{x \in \mathcal{C}_k} \dfrac{1}{2} p^\top \Big(\Sigma_x - \Sigma_x L (I_r + L^\top\Sigma_x L)^{-1} L^\top \Sigma_x \Big) p \\
\end{align*}
where $\Sigma_u = D^{-1/2} \diag(u) D^{-1/2}$.  Reformulating the problem as a min and introducing a slack variable the result follows.
\end{proof}

\begin{lemma}
Another bidual of \eqref{eq:dual-eqcons} is 
\begin{align*}
    \min_{\substack{z \\ u \in [0,1]^m \\ \ones^\top u \leq k}} \dfrac{1}{2} p^\top \Sigma_u p + \dfrac{1}{2}\|z\|_2^2 + \dfrac{1}{2}(z + L\Sigma_u p)^\top (L^\top \Sigma_u L)^{-1} (z + L\Sigma_u p)
\end{align*}
where $\Sigma_u = \Lambda^{1/2} \diag(u) \Lambda^{1/2}$
\end{lemma}
\begin{proof}
For visual clarity, we write $d^\ast(k)$ as $d^\ast$ and $p^{\ast \ast}(k)$ as $p^{\ast \ast}$.
Starting from \eqref{eq:dual-eqcons}
\begin{align*}
    d^\ast = \max_{\nu,y} -\dfrac{1}{2}\|\nu\|_2^2 -s_k(y \circ y) \; : \; y = \tfrac{1}{\sqrt{2}}\Lambda^{-1/2} (p + L\nu)
\end{align*}
we note that
\begin{align*}
    s_k(y \circ y) = \max_{\substack{u \in [0,1]^m \\ \ones^\top u \leq k}} y^\top \diag(u) y
\end{align*}
Now using the variational form of $s_k(\cdot)$ given above along side the Fenchel conjugate of a quadratic, our bidual reads
\begin{align*}
    -p^{\ast \ast} = -d^\ast &= \min_{\nu,y} \max_{\substack{z \\ u \in [0,1]^m \\ \ones^\top u \leq k}} \nu^\top z - \dfrac{1}{2}\|z\|_2^2 + y^\top \diag(u) y \; : \; y = \tfrac{1}{\sqrt{2}}\Lambda^{-1/2} (p + L\nu) \\
    &= \max_{\substack{z \\ u \in [0,1]^m \\ \ones^\top u \leq k}} -\dfrac{1}{2} \|z\|_2^2 + \min_{\nu, y} \nu^\top z + y^\top \diag(u) y \; : \; y = \tfrac{1}{\sqrt{2}}\Lambda^{-1/2} (p + L\nu)
\end{align*}
where the last equality holds because of strong duality. The minimization over $y$ is trivial and the minimization over $\nu$ can be done in closed form to arrive at
\begin{align*}
    -p^{\ast \ast} = \max_{\substack{z \\ u \in [0,1]^m \\ \ones^\top u \leq k}} - \dfrac{1}{2}p^\top \Sigma_u p -\dfrac{1}{2} \|z\|_2^2  - \dfrac{1}{2} (z + L^\top \Sigma_u p)^\top (L^\top \Sigma_u L)^{-1} (z + L^\top \Sigma_u p)
\end{align*}
where $\Sigma_u = \Lambda^{-1/2} \diag(u) \Lambda^{-1/2}$.
\end{proof}

We now use the Shapley Folkman theorem to show that problem~\eqref{eq:BD-QP} has a solution with at most XXX nonbinary variables $u_i$ among the $m$ problem variables $u\in[0,1]^m$.

\begin{lemma}
The interval relaxation of \eqref{eq:primal-sdp}, namely
\begin{align}
    p^{\ast \ast}(k) = &\min_{u \in [0,1]^m} \; \tfrac{1}{2}t \tag{BD-QP} \\
    \text{s.t} & \hspace{5mm} \begin{bmatrix}
    t + p^\top \Sigma_x p & p^\top \Sigma_x L  \\
    L^\top \Sigma_x p & I_r + L^\top \Sigma_x L 
    \end{bmatrix} \succeq 0 \nonumber \\
    & \hspace{5mm} \Sigma_x = \Lambda^{1/2} \diag(u) \Lambda^{1/2} \nonumber \\
    & \hspace{5mm} \ones^\top u \leq k \nonumber
\end{align}
has a solution with at most $r(r+1)/2+2$ nonbinary coefficients $u_i$, i.e. $\Card(\{u_i \notin {0,1}\})\leq r(r+1)/2+2$.
\end{lemma}
\begin{proof}
We can write problem~\eqref{eq:primal-sdp} in the form
\[\BA{ll}
\mbox{min.} & \tfrac{1}{2}t\\
\mbox{s.t.} & 
\begin{bmatrix}
    t & 0  \\
    0 & I_r  
\end{bmatrix}
+ \displaystyle \sum_{i=1}^m
\begin{bmatrix}
    p^\top \Lambda^{1/2} \diag(u) \Lambda^{1/2} p & \diag(p) \Lambda L  \\
    L^\top \Lambda \diag(u) p &  L^\top \Lambda^{1/2} \diag(u) \Lambda^{1/2} L 
    \end{bmatrix} \in \symm_+^{k+1}\\
    &  \ones^\top u \leq k 
\EA\]
in the variables $t \in \reals ,u\in[0,1]^m$. This is also
\[\BA{ll}
\mbox{min.} & \tfrac{1}{2}t\\
\mbox{s.t.} & 
\begin{bmatrix}
    t & 0 & 0 \\
    0 & I_r & 0\\
    0 & 0 & k
\end{bmatrix}
+ \displaystyle \sum_{i=1}^m u_i
\begin{bmatrix}
    \lambda_i p_i^2 & V_i^\top & 0\\
    V_i  & W_i W_i^\top & 0\\
    0 & 0 & -1
    \end{bmatrix} \in \symm_+^{k+1}\\
\EA\]
where we have written $V=L^\top \Lambda \diag(p)$ and $W=L^\top \Lambda^{1/2}$. This can be rewritten in a more geometric format
\[\BA{ll}
\mbox{min.} & \tfrac{1}{2}t\\
\mbox{s.t.} & 
\left\{\begin{bmatrix}
    t & 0 & 0 \\
    0 & I_r & 0\\
    0 & 0 & k
\end{bmatrix}
+ \displaystyle \sum_{i=1}^m 
\Co\left(\left\{0,
\begin{bmatrix}
    \lambda_i p_i^2 & V_i^\top & 0\\
    V_i  & W_i W_i^\top & 0\\
    0 & 0 & -1
    \end{bmatrix} 
    \right\}\right)\right\}~
    \bigcap ~ \symm_+^{k+1} \neq \emptyset\\
\EA\]
Now, the Shapley Folkman theorem \citep{Star69} states that if 
\[
x \in \sum_{i=1}^m 
\Co\left(\left\{0,
\begin{bmatrix}
    \lambda_i p_i^2 & V_i^\top & 0\\
    V_i  & W_i W_i^\top & 0\\
    0 & 0 & -1
    \end{bmatrix} 
    \right\}\right)
\]
then 
\[
x \in \sum_{i\in \mathcal{S}}
\Co\left(\left\{0,
\begin{bmatrix}
    \lambda_i p_i^2 & V_i^\top & 0\\
    V_i  & W_i W_i^\top & 0\\
    0 & 0 & -1
    \end{bmatrix} 
    \right\}\right)
    + \sum_{i\in \mathcal{S}^c}
\left\{0,
\begin{bmatrix}
    \lambda_i p_i^2 & V_i^\top & 0\\
    V_i  & W_i W_i^\top & 0\\
    0 & 0 & -1
    \end{bmatrix} 
    \right\}
\]
where $|\mathcal{S}|\leq r(r+1)/2+2$, because the matrices belong to a subspace of dimension $r(r+1)/2+1$.
\end{proof}







==> dual_clean.tex <==
%!TEX root = nonlin.tex
\section{Dual}
\label{sec:dual}

\subsection{Primal Reformulation}
We introduce two reformulations of the primal problem \eqref{eq:primal} that are equivalent to each other.
\begin{lemma} \label{lem:equiv}
\begin{align}\label{eq:primal-eqcons}
    p^\ast(k) = &\min_{z, \|x\|_0 \leq k} \; \dfrac{1}{2}x^\top \Lambda x + \dfrac{1}{2} z^\top z + p^\top x  \tag{P1} \\
    \text{s.t} & \hspace{5mm} L^\top x = z \nonumber
\end{align}
and
\begin{align}\label{eq:primal-mm}
    p^\ast(k) = \min_{\substack{v \in \mathbb{R}^r, u \in \{0,1\}^m \\ \ones^\top u \leq k}} \dfrac{1}{2} p^\top \Sigma_u p + \dfrac{1}{2}v^\top (I_r + L^\top \Sigma_u L ) v - v^\top L^\top \Sigma_u p  \tag{P2}\\
\end{align}
\end{lemma}
\begin{proof}
The equivalence between \eqref{eq:primal} and \eqref{eq:primal-eqcons} follows immediately. To arrive at \eqref{eq:primal-mm}, we start from \eqref{eq:primal} and make the variable substitution $x = \diag(u) v $ where $v \in \mathbb{R}^m$ and $u \in \{0,1\}^m$ with $\ones^\top u \leq k$. We then have
\begin{align}\label{eq:primal-boolean}
    p^\ast(k) = \min_{\substack{u \in \{0,1\}^m \\ \ones^\top u \leq k}} \min_v \dfrac{1}{2}v^\top \diag(u) \Big( \Lambda + LL^\top \Big) \diag(u) v + p^\top \diag(u) v
\end{align}
We first compute the inner minimization over $v$. Note that at optimum, the sparsity pattern of $v$ must follow that of $u$ since $\Lambda \succ 0$. As a result, $v^\top \diag(u) \Lambda \diag(u) v = v^\top \Lambda v$. Setting the gradient with respect to $v$ equal to 0, we find that
\begin{align*}
    v^\ast = -\Big(\Lambda + \diag(u) LL^\top \diag(u)\Big)^{-1} \diag(u)p
\end{align*}
and after substituting back into the objective and using the fact that $(\diag(u))^2 = \diag(u^2)$ and the Woodbury matrix identity
\begin{align*}
\Big(\Lambda + \diag(u) LL^\top \diag(u)\Big)^{-1} = \Lambda^{-1} - \Lambda^{-1} \diag(u) L \Big(I_k + L^\top \diag(u) L\Big)^{-1} L^\top \diag(u) \Lambda^{-1}
\end{align*}
we have that
\begin{align*}
    p^\ast(k) = \min_{\substack{u \in \{0,1\}^m \\ \ones^\top u \leq k}} \dfrac{1}{2}p^\top \Big(\Sigma_u - \Sigma_u L(I_r + L^\top \Sigma_u L)^{-1} L^\top \Sigma_u \Big) p
\end{align*}
where $\Sigma_u = \Lambda^{1/2} \diag(u) \Lambda^{1/2}$. Note additionally that
\begin{align*}
    p^\ast(k) &= \min_{\substack{v \in \mathbb{R}^r, u \in \{0,1\}^m \\ \ones^\top u \leq k}} \dfrac{1}{2} p^\top \Sigma_u p + \dfrac{1}{2}v^\top (I_r + L^\top \Sigma_u L ) v - v^\top L^\top \Sigma_u p  
    % &= \min_{\substack{v \in \mathbb{R}^r, u \in \{0,1\}^m \\ \ones^\top u \leq k}} \dfrac{1}{2}\sum_{i=1}^m \; u_i \Big[(1 + \lambda_i)(\ell_i^\top v)^2 - (\lambda_i p_i) (\ell_i^\top v) \Big]\\
\end{align*}
\end{proof}

\subsection{Dual problem}
While both formulations are equivalent, we concern ourselves with the dual of \eqref{eq:primal-eqcons} since it is simpler to compute.

\begin{lemma}
The dual of \eqref{eq:primal-eqcons} is
\begin{align}\label{eq:dual-eqcons}
    d^\ast(k) = \max_\nu \left\{-\dfrac{1}{2} \|\nu\|_2^2 - s_k\left(\tfrac{1}{2\lambda_{i}} (p_i + \ell_i^\top \nu)^2\right)\right\} \tag{D-P1} \nonumber
\end{align}
where $s_k(\cdot)$ is the sum of the top $k$ entries of a vector.
\end{lemma}

\begin{proof}
For visual clarity, we rewrite $d^\ast(k)$ as $d^\ast$ throughout the proof. Dualizing the equality constraint we have
\begin{align*}
d^\ast = \max_{\nu}  g(\nu)
\end{align*}
where
\begin{align*}
g(\nu) = \min_{z, \|x\|_0 \leq k} \;\; \dfrac{1}{2} x^\top \Lambda x + \dfrac{1}{2}\|z\|_2^2 + p^\top x + \nu^\top(L^\top x - z)
\end{align*}
The minimization over $z$ is trivial: $z^\ast = \nu$. Hence we arrive at
\begin{align*}
d^\ast = \max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 +   \min_{\|x\|_0 \leq k}  \dfrac{1}{2} x^\top \Lambda x  + x^\top (p + L\nu)
\end{align*}
Introducing an index set $\mathcal{I}$ such that $\mathcal{I} \subseteq \{1,\hdots,m\}$ and $|\mathcal{I} | \leq k$ and on $\mathcal{I}^C$ we have $x = 0$. Letting $\lambda_i = \Lambda_{ii}$ and letting $\ell_i^\top$ denote the $i$th row of $L$, we have that
\begin{align*}
d^\ast &= \max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 +   \min_{\mathcal{I} \subseteq \{1,\hdots,n\}, |\mathcal{I}| \leq k} \min_x \;  \sum_{i \in \mathcal{I}} \; \dfrac{1}{2}\lambda_i x_i^2  + x_i (p_i + \ell_i^\top \nu) + \sum_{i \in \mathcal{I}^C} 0 \\
&= \max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 +   \min_{\mathcal{I} \subseteq \{1,\hdots,n\}, |\mathcal{I}| \leq k} \;  \sum_{i \in \mathcal{I}} \; \min_{x_i} \dfrac{1}{2}\lambda_i x_i^2  + x_i (p_i + \ell_i^\top \nu) + \sum_{i \in \mathcal{I}^C} 0 
\end{align*}
Solving the inner minimization over $x_i$ we have that
\begin{align*}
d^\ast &= \max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 +   \min_{\mathcal{I} \subseteq \{1,\hdots,n\}, |\mathcal{I}| \leq k} \;  \sum_{i \in \mathcal{I}}  -\dfrac{1}{2\lambda_i} (p_i + \ell_i^\top \nu)^2 + \sum_{i \in \mathcal{I}^C} 0 
\end{align*}
We can rewrite the optimization over $\mathcal{I}$ equivalently as 
\begin{align*}
\min_{\mathcal{I} \subseteq \{1,\hdots,n\}, |\mathcal{I}| \leq k} \;  \sum_{i \in \mathcal{I}}  -\dfrac{1}{2\lambda_i} (p_i + \ell_i^\top \nu)^2 + \sum_{i \in \mathcal{I}^C} 0  = \min_{u \in \{0,1\}^n, \; \textbf{1}^\top u \leq k} \; u^\top \alpha + (1-u)^\top 0
\end{align*}
where $\alpha_i = -\tfrac{1}{2\lambda_i} (p_i + \ell_i^\top \nu)^2$. Hence we have
\begin{align*}
-d^\ast &= -\max_{\nu} -\dfrac{1}{2} \|\nu\|_2^2 + \min_{u \in \{0,1\}^n, \; \textbf{1}^\top u \leq k} \; u^\top \alpha  \\
&= \min_{\nu} \dfrac{1}{2} \|\nu\|_2^2 - \max_{u \in \{0,1\}^n, \; \textbf{1}^\top u \leq k} \; -u^\top \alpha
\end{align*}
Note the inner minimization reduces to the sum of the top $k$ entries of $-\alpha$ and hence the problem writes
\begin{align*}
-d^\ast = -\min_\nu \dfrac{1}{2} \|\nu\|_2^2 + s_k(-\alpha)
\end{align*}
where $s_k( \cdot)$ denotes the sum of the top $k$ entries of a vector. The dual problem is (as expected) convex.
\end{proof}

\subsection{Bidual problem}
We now compute the bidual of \eqref{eq:dual-eqcons} and show that it is equivalent to the interval relaxation of \eqref{eq:primal-mm}.
\begin{lemma}
A dual of \eqref{eq:dual-eqcons} (i.e. a bidual of \eqref{eq:primal-eqcons}) is equivalent to the interval relaxation of \eqref{eq:primal-mm}, namely
\begin{align}\label{eq:BD-QP}
    p^{\ast \ast}(k) = \min_{\substack{v \in \mathbb{R}^r, u \in [0,1]^m \\ \ones^\top u \leq k}} \dfrac{1}{2} p^\top \Sigma_u p + \dfrac{1}{2}v^\top (I_r + L^\top \Sigma_u L ) v - v^\top L^\top \Sigma_u p  \tag{BD-P2}\\
\end{align}
\end{lemma}
\begin{proof}
For visual clarity, we write $d^\ast(k)$ as $d^\ast$ and $p^{\ast \ast}(k)$ as $p^{\ast \ast}$ throughout the proof. Note that
\begin{align*}
s_k(c) = \min_{\lambda \geq 0} \; \lambda k + \sum_{i=1}^n \max(0, c_i - \lambda)
\end{align*}
and the dual of $s_k(\cdot)$ can be written as 
\begin{align*}
\max_{x \in [0,1]^m} x^\top c \;\; : \;\; \textbf{1}^\top x \leq k 
\end{align*}
where we introduce a slack variable for the $\max(0,c_i - \lambda)$ term, dualize using two dual variables, and then eliminate one of the dual variables.
Using this we have that
\begin{align*}
-p^{\ast\ast} = -d^\ast = \min_\nu \max_{u \in \mathcal{C}_k} \dfrac{1}{2} \|\nu\|_2^2 - u^\top \alpha 
\end{align*}
where $\mathcal{C}_k = \{ u \; | \; \textbf{1}^\top x \leq k, \; x \in [0,1]^m \}$. By Sion's minimiax theorm, we can exchange the min and max to arrive at
\begin{align*}
-p^{\ast \ast} = \max_{u \in \mathcal{C}_k} \min_\nu  \dfrac{1}{2} \|\nu\|_2^2 - u^\top \alpha 
\end{align*}
Note that $u^\top \alpha = -\dfrac{1}{2}(p + L\nu)^\top \Lambda^{-1/2} \diag(u) \Lambda ^{-1/2} (p+L\nu)$ where $\diag(u) = \diag(u_1,\hdots,u_m)$ . Taking the minimization over $\nu$ we have
\begin{align*}
\nu^\ast = (I + L^\top D^{-1/2} \diag(u) D^{-1/2} L)^{-1} L^\top D^{-1/2} \diag(u) D^{-1/2} p
\end{align*}
Plugging back in, our objective reduces to
\begin{align*}
-p^{\ast \ast} = \max_{x \in \mathcal{C}_k} -\dfrac{1}{2} p^\top \Big(\Sigma_x - \Sigma_x L (I_r + L^\top\Sigma_x L)^{-1} L^\top \Sigma_x \Big) p \\
\end{align*}
where $\Sigma_u = D^{-1/2} \diag(u) D^{-1/2}$.  Reformulating the problem as a min using the same eqeuivalence as in Lemma \ref{lem:equiv} the result follows.
\end{proof}








==> dualsocp.tex <==
%!TEX root = main.tex
\section{Conic Dual}
\label{sec:dualsocp}

\subsection{Constrained Problem}\label{ss:l1-const-prob}

We focus on the following optimization problem
\BEQ\label{eq:socp}\tag{SOCP}
\BA{rll}
p^\star(k) =& \mbox{min.} & x^\top \Lambda x + z^\top z + 2 p^\top x\\
&\mbox{subject to} & L^\top x =z \\
&& \|x\|_0 \leq k, ~\|x\|_\infty \leq \beta,\\
\EA\EEQ
in the variables $x\in\reals^m$, $z\in\reals^r$, where $\beta>0$. We cast this problem using SOCP constraints, written
\[
\BA{ll}
\mbox{minimize} &  t +  v \\
\mbox{subject to} & L^\top x =z \\
& \left\|\left(\Lambda^{1/2} x,(1+2p^\top x -t)/2\right)\right\| \leq (1-2 p^\top x +t)/2\\
& \left\|\left(z,(1 -v)/2\right)\right\| \leq (1+v)/2\\
& \|x\|_0 \leq k, ~\|x\|_\infty \leq \beta,\\
\EA\]
% using the fact
% \begin{align*}
%     u^\top u \leq yz, \; y \geq 0, \; z \geq 0 \Longleftrightarrow \bigg\| \begin{bmatrix}
%     2u \\
%     y - z
%     \end{bmatrix} \bigg\|_2 \leq y + z, \; y \geq 0, \; z \geq 0
% \end{align*}
using the fact that 
\[
\|(1+t)/2,Ax)\|\leq (1-t)/2 
\Longleftrightarrow
x^\top A^\top Ax +t \leq 0.
\]
We write $\mathcal{K}_2$ the second order cone, with
\[
\mathcal{K}_2\triangleq \left\{(t,y)\in\reals^{n+1}:\|y\|_2\leq t\right\}.
\]

\subsubsection{Dual} Because $\mathcal{K}_2$ is a symmetric cone, i.e. $\mathcal{K}_2^*=\mathcal{K}_2$, the dual of this last problem is given by 
\BEAS
\max_{\substack{\chi,\mu,\in\mathcal{K}_2\\\nu\in\reals^r}}~\min_{\substack{z,t,v,\|x\|_0 \leq k,\\ \|x\|_\infty \leq \beta,}} &&  t +  v + \nu^\top (L^\top x-z) - \mu_1(1-2 p^\top x +t)/2 -\mu_2 (1+ 2p^\top x -t)/2 -\mu_3^\top \Lambda^{1/2} x\\
&& - \chi_1(1+v)/2 - \chi_2(1-v)/2 -\chi_3^\top z
\EEAS
in the variables $\chi=(\chi_1,\chi_2,\chi_3),\mu=(\mu_1,\mu_2,\mu_3),\in\mathcal{K}_2$, with $\chi_1,\chi_2,\mu_1,\mu_2\in\reals$, and $\nu\in\reals^r$. Minimizing over $t,v,z$, this reduces to
\[
\max_{\substack{\chi,\mu,\in\mathcal{K}_2\\\mu_1-\mu_2=2,\\\chi_1-\chi_2=2}}~\min_{\substack{\|x\|_0 \leq k,\\ \|x\|_\infty \leq \beta}} ~ (2 p - L \chi_3 -  \Lambda^{1/2} \mu_3)^\top x - (\mu_1 + \mu_2 + \chi_1 + \chi_2)/2
\]
and the dual then becomes
\BEQ\label{eq:dual-socp}\tag{Dual-SOCP}
\max_{\substack{\chi,\mu,\in\mathcal{K}_2\\\mu_1-\mu_2=2,\\\chi_1-\chi_2=2}}~ - \beta \,s_k(|2 p - L \chi_3 -  \Lambda^{1/2} \mu_3|) - (\mu_1 + \mu_2 + \chi_1 + \chi_2)/2
\EEQ
in the variables $\chi, \mu\in\mathcal{K}_2$, with 
\BEQ\label{def:sk-abs}
s_k(|y|)\triangleq \max_{\substack{\|x\|_0 \leq k,\\ \|x\|_\infty \leq 1}} x^\top |y|
~ = ~  
\max_{\substack{\|x\|_1 \leq k ,\\ \|x\|_\infty \leq 1}} x^\top |y| 
\EEQ
where $|y|$ is the vector whose coefficients are equal to $|y_i|$. Using this last equivalence between $\ell_0$ and $\ell_1$ variational formulations of $s_k(|\cdot|)$, we can form the bidual of problem~\eqref{eq:socp} as
\BEAS
\max_{\substack{\chi,\mu,\in\mathcal{K}_2\\\nu\in\reals^r}}~\min_{\substack{z,t,v,\|x\|_1 \leq \beta k,\\ \|x\|_\infty \leq \beta,}} &&  t +  v + \nu^\top (L^\top x-z) - \mu_1(1-2 p^\top x +t)/2 -\mu_2 (1+ 2p^\top x -t)/2 -\mu_3^\top \Lambda^{1/2} x\\
&& - \chi_1(1+v)/2 - \chi_2(1-v)/2 -\chi_3^\top z
\EEAS
for which strong duality holds by compactness and convexity. The bidual thus reads
\BEQ\label{eq:bidual-socp}
\BA{rll}
d^\star(k) = & \mbox{min.} & x^\top \Lambda x + z^\top z + 2 p^\top x\\
&\mbox{subject to} & L^\top x =z \\
&& \|x\|_1 \leq k\beta, ~\|x\|_\infty \leq \beta\\
\EA\EEQ
in the variables $x\in\reals^m$, $z\in\reals^r$. This Lagrangian relaxation is simply the $\ell_1$ relaxation of problem~\eqref{eq:socp}.


\subsubsection{Duality Gap Bounds}
We first recall some key results from \citep{Ekel99} on the Shapley Folkman theorem and a priori duality gap bounds. Given functions $f_i$, a vector $b \in \reals^m$, and vector-valued functions $g_i$, $i\in[n]$ that take values in $\reals^m$, consider the following problem: 
\BEQ\label{eq:p-ncvx-pb-const}\tag{OPT}
\mathrm{h}_{P}(u) := \min_x \: \sum_{i=1}^{n} f_i(x_i) ~:~ \sum_{i = 1}^n g_i(x_i) \leq b + u,
\EEQ
in the variables $x_i\in\reals^{d_i}$, with perturbation parameter $u\in\reals^m$. We now recall some basic definitions on conjugate functions and convex envelopes. 

\paragraph{Biconjugate, convex envelope \& Lack of Convexity.}
Given a function $f$, not identically $+\infty$, minorized by an affine function, we write
\[
f^*(y)\triangleq \inf_{x\in\dom f} \{y^{\top}x - f(x)\}
\]
the conjugate of $f$, and $f^{**}(y)$ its biconjugate. The biconjugate of $f$ (aka the convex envelope of $f$) is the pointwise supremum of all affine functions majorized by $f$ (see e.g. \citep[Th.\,12.1]{Rock70} or \citep[Th.\,X.1.3.5]{Hiri96}), a corollary then shows that $\epi(f^{**})=\overline{\Co(\epi(f))}$. For simplicity, we write $S^{**}=\overline{\Co(S)}$ for any set $S$ in what follows. We will make the following technical assumptions on the functions $f_i$ and $g_i$ in our problem.
\begin{assumption}\label{as:fi}
The functions $f_i: \reals^{d_i} \rightarrow \reals$ are proper, 1-coercive, lower semicontinuous and there exists an affine function minorizing them.
\end{assumption}
Note that coercivity trivially holds if $\dom(f_i)$ is compact (since $f$ can be set to $+\infty$ outside w.l.o.g.). When Assumption~\ref{as:fi} holds, $\epi(f^{**})$, $f_i^{**}$ and hence $\sum_{i=1}^{n} f_i^{**}(x_i)$ are closed \citep[Lem.\,X.1.5.3]{Hiri96}. Also, as in e.g. \citep{Ekel99}, we define the lack of convexity of a function as follows.

\begin{definition}\label{def:rho}
Let $f: \reals^{d} \rightarrow \reals$, we let 
\BEQ\label{eq:rho}
\rho(f)\triangleq \sup_{x\in \dom(f)} \{f(x) - f^{**}(x)\}
\EEQ
\end{definition}

Many other quantities measure lack of convexity (see e.g. \citep{Aubi76,Bert14} for further examples). In particular, the nonconvexity measure $\rho(f)$ can be rewritten as
\BEQ\label{def:alt-lack-cvx}
\rho(f)=\sup_{\substack{x_i\in \dom(f)\\ \mu\in\reals^{d+1}}}~\left\{ f\left(\sum_{i=1}^{d+1}\mu_i x_i\right) -  \sum_{i=1}^{d+1}\mu_i f(x_i): \ones^\top \mu=1,\mu \geq 0\right\}
\EEQ
when $f$ satisfies Assumption~\ref{as:fi} (see \citep[Th.\,X.1.5.4]{Hiri96}).


\paragraph{Bounds on the duality gap and the Shapley-Folkman Theorem}
Let $\mathrm{h}_{P}(u)^{**}$ be the biconjugate of $\mathrm{h}_{P}(u)$ defined in~\eqref{eq:p-ncvx-pb-const}, then $\mathrm{h}_{P}(0)^{**}$ is the optimal value of the dual to~\eqref{eq:p-ncvx-pb-const} \citep[Lem.\,2.3]{Ekel99}, and \citep[Th.\,I.3]{Ekel99} shows the following result.

\begin{theorem}\label{th:sf}
Suppose the functions $f_i,g_{ji}$ in problem~\eqref{eq:p-ncvx-pb-const} satisfy Assumption~\ref{as:fi} for $i=1,\ldots,n$, $j=1,\ldots,m$. Let
\BEQ\label{eq:sf-pbar}
\bar p_j = (m+1) \max_i \rho(g_{ji}), \quad \mbox{for $j=1,\ldots,m$}
\EEQ
then 
\BEQ\label{eq:sf-bnd}
\mathrm{h}_{P}(\bar p) \leq \mathrm{h}_{P}(0)^{**} + (m+1)\max_i \rho(f_i).
\EEQ
where $\rho(\cdot)$ is defined in Def.~\ref{def:rho}.
\end{theorem}

This last result directly translates into a bound on the duality gap of problem~\eqref{eq:socp}.

\begin{proposition}\label{eq:gap-socp}
Let $p^\ast(k)$ and $d^\ast(k)$ be defined as in \eqref{eq:socp} and \eqref{eq:dual-socp} respectively, then
\BEQ\label{eq:sf-bnd}
   p^\star(k + (r+2)) \leq d^\star(k) \leq p^\star (k) \leq d^\star (k - (r+2))
\EEQ
where $k \geq (r+2)$.
\end{proposition}\label{prop:sfs-socp}
\begin{proof}
Since the objective in \eqref{eq:primal-eqcons} is separable, we can write the problem in perturbation form as
\begin{align*}
    h_P(u) = &\min_{\|x\|_\infty\leq\infty,z} \; \dfrac{1}{2}x^\top \Lambda x + \dfrac{1}{2} z^\top z + p^\top x  \tag{P-QP} \\
    \text{s.t} & \hspace{5mm} L^\top x = z + u_1 \nonumber \\
     & \hspace{5mm} \sum_{i=1}^m  \ones_{x_i \not = 0} \leq k + u_2 \nonumber
\end{align*}
where $u=(u_1,u_2) \in \mathbb{R}^{r + 1}$ is a perturbation vector. By construction, we have $d^\star(k) = -h_P(0)$ and $d^\star(k + l) = -h_P((0,l))$. Note that the function $\ones_{x_i \not = 0}$ is lower semicontinuous and that all functions in question are 1-coercive, hence satisfy Assumption 1 above. We can bound the lack of convexity of $\ones_{x_i \not = 0}$ for all $i$ by 1 on $\|x\|_\infty\leq \beta$ with
\begin{align*}
    \rho(\ones_{x \not = 0}) = \sup_{\|x\|_\infty \leq \beta} \ones_{x \not = 0} - |x|/\beta = 1
\end{align*}
This means  that $\max_i \rho(g_{ji}) = 1$ in Theorem \ref{th:sf} (the lack of convexity measure for the equality constraints are 0). Hence our perturbation vector $\bar{p} = (0, 1)$. Because there are $r+1$ constraints in \eqref{eq:socp} (the constraints $\|x\|\leq \infty$ are not coupling), we have 
\[
    h_P(\bar{p}) = h_P((0,(r+2))) = d^\star(k + (r+2))
\]
The objective function being convex and separable, $\max_i \rho(f_i) = 0$ and Theorem \ref{th:sf} yields
\[
    p^\star(k + \lfloor (r+2)\rfloor) \leq d^\star(k)
\]
The other bound follows immediately from weak duality.
\end{proof}

Note that this bound on the duality gap depends on the rate of growth of $p^\star(k)$, it is in particular tighter in regions where this function is relatively flat, i.e. where increasing $k$ means adding somewhat irrelevant features.


\subsubsection{Primalization}
While the equivalence in~\eqref{def:sk-abs} holds in objective values, the solutions' support can vary significantly between $\ell_1$ and $\ell_0$ formulation. In what follows, we show how to extract a feasible point satisfying the bound~\eqref{eq:sf-bnd} from an optimal point of the relaxation~\eqref{eq:dual-socp}. 

\begin{proposition}\label{prop:prim}
Suppose $x\in\reals^m$ and $z\in\reals^r$ solve~\eqref{eq:dual-socp}, and form the following linear feasibility problem
\BEQ\label{eq:lp}
\BA{rcl}
d^\star(k) & \geq & z^\top z + \sum_{i=1}^m \mu_i (x_i^2 \lambda_i +2 p_i x_i) \\
0 & = & z - \sum_{i=1}^m \mu_i x_i L_i  \\
k & \geq & \sum_{i=1}^m \mu_i\\
0 & \leq & \mu \\
1 & \geq & \mu
\EA\EEQ
in the variables $\mu\in\reals^m$.
\end{proposition}




\subsection{Penalized problem}\label{ss:l1-pen-prob}
We now focus on the following penalized optimization problem
\BEQ\label{eq:lasso-l0}\tag{PQP}
\BA{rll}
p^\star(\gamma) =& \mbox{min.} & \tfrac{1}{2} x^\top \Lambda x + \tfrac{1}{2} z^\top z + p^\top x + \gamma \|x\|_0\\
&\mbox{subject to} & L^\top x =z \\
\EA\EEQ
in the variables $x\in\reals^m$, $z\in\reals^r$, where $\gamma>0$. This penalized formulation of this sparse quadratic program, akin to LASSO, is separable in $x$ and we can write it 
\[\BA{rll}
p^\star(\gamma) =& \mbox{min.} & \sum_{i=1}^m ( \tfrac{1}{2}\lambda_i x_i^2 + p_i x_i + \gamma \ones_{\{x_i\neq 0\}}) + \tfrac{1}{2}z^\top z \\
&\mbox{subject to} & L^\top x =z \\
\EA\]
in the variables $x\in\reals^m$, $z\in\reals^r$, where $\gamma>0$. As in \citep{Udel16}, we can write a convex relaxation of this problem using the convex envelope of the function $f_i(x)= \tfrac{1}{2}\lambda_i x_i^2 + p_i x_i + \gamma \ones_{\{x_i\neq 0\}}$, given in e.g. \citep{Soub15}
\BEQ\label{eq:fhat}
\hat f_i(x,\gamma) \triangleq  \dfrac{1}{2}\lambda_i x_i^2 + p_i x_i + \gamma - \dfrac{\lambda_i}{2} \left(|x|-\sqrt{\frac{2\gamma}{\lambda_i}}\right)^2 \ones_{\left\{|x|\leq \sqrt{{2\gamma}/{\lambda_i}} \right\}}
\EEQ
Using the fact that the conjugate is linear with respect to the sum of separable functions, a convex relaxation of~\eqref{eq:lasso-l0} reads
\BEQ\label{eq:lasso-relax}
\BA{rll}
d^\star(\gamma) =& \mbox{min.} & \sum_{i=1}^m \hat f_i(x,\gamma) + \tfrac{1}{2} z^\top z \\
&\mbox{subject to} & L^\top x =z \\
\EA\EEQ
in the variables $x\in\reals^m$, $z\in\reals^r$, where $\gamma>0$.

\subsubsection{Dual of \eqref{eq:lasso-l0}}
The lagrange relaxation of \eqref{eq:lasso-l0} reads
\begin{align*}
    d^\ast (\gamma) = \max_\nu \min_{x,z} \sum_{i=1}^m (\lambda_i x_i^2 + 2p_i x_i + \gamma \ones_{\{x_i\neq 0\}}) + z^\top z + \nu^\top (z - L^\top x)
\end{align*}
The minimization over $z$ gives $z^\ast = -\nu/2$. Since the problem in separable in $x$, for each $i$ we have that $x_i^\ast =  -\tfrac{1}{2\lambda_i} (2p_i + \ell_i^\top \nu)$ if $\alpha_i := -\tfrac{1}{4\lambda_i} (2p_i + \ell_i^\top \nu)^2 < -\gamma$ and $x_i^\ast = 0$ otherwise. The dual problem then simplifies to
\begin{align}\label{eq:lasso-l0-dual}\tag{D-PQP}
    d^\ast(\gamma) = \max_\nu -\dfrac{1}{4}\|\nu\|_2^2 + \sum_{i=1}^m \min(0, \alpha_i + \gamma)
\end{align}

\subsubsection{Bidual of \eqref{eq:lasso-l0}}
Starting from \eqref{eq:lasso-l0-dual}, and using the fact that
\begin{align*}
    \min(x,y) = \min_{s \in [0,1]} (1-s)x + sy
\end{align*}
we have via strong duality that
\begin{align*}
    p^{\ast \ast}(\gamma) &= \max_\nu \min_{s \in [0,1]^m} -\dfrac{1}{4}\|\nu\|_2^2 + \sum_{i=1}^m s_i(\alpha_i + \gamma ) \\
    &=\min_{s \in [0,1]^m} \max_\nu  -\dfrac{1}{4}\|\nu\|_2^2 + s^\top \alpha + \gamma \ones^\top s
\end{align*}
Note that $s^\top \alpha = -\dfrac{1}{4}(2p + L\nu)^\top \Lambda^{-1/2} \diag(s) \Lambda ^{-1/2} (2p+L\nu)$ where $\diag(s) = \diag(s_1,\hdots,s_m)$ . Taking the maximization over $\nu$ we have
\begin{align*}
    \nu^\ast = -2(I_r + L^\top \Lambda^{-1/2} \diag(s) \Lambda ^{-1/2}L)^{-1} L^\top \Lambda^{-1/2} \diag(s) \Lambda ^{-1/2} p
\end{align*}
Plugging back in our objective reduces to
\begin{align*}
p^{\ast \ast}(\gamma) = \min_{s \in [0,1]} -\dfrac{1}{4} p^\top \Big(\Sigma_s - \Sigma_s L (I_r + L^\top\Sigma_s L)^{-1} L^\top \Sigma_s \Big) p  + \gamma \ones^\top s
\end{align*}
where $\Sigma_s = \Lambda^{-1/2} \diag(s) \Lambda^{-1/2}$.  


\paragraph{Bounds on the duality gap and the Shapley-Folkman Theorem}

Let $\rho(\hat f)$ be the lack of convexity of the function as defined in~\eqref{eq:rho}. We have the following lemma.

\begin{lemma}\label{lem:rho-fhat}
The lack of convexity of the function $f_i$ satisfies 
\BEQ\label{rho-fhat}
\rho(\hat f_i) \leq \gamma
\EEQ
\end{lemma}
\begin{proof}
We have 
\[
\rho(\hat f_i) = \sup_x \left\{\gamma \ones_{\{x_i\neq 0\}}- \gamma + \lambda_i \left(|x|-\sqrt{\frac{\gamma}{\lambda_i}}\right)^2 \ones_{\left\{|x|\leq \sqrt{{\gamma}/{\lambda_i}} \right\}}\right\} \leq \gamma.
\] 
\end{proof}

The a priori bounds on the duality gap derived from the Shapley-Folkman theorem then yield the following result.


\begin{proposition}
We have
\BEQ\label{eq:bnd-pen}
d^\star(\gamma) \leq p^\star(\gamma) \leq d^\star(\gamma) + \gamma (r+1).
\EEQ
where $p^\star(\gamma)$ is the optimum of problem~\eqref{eq:lasso-l0} and $d^\star(\gamma)$ that of~\eqref{eq:lasso-relax}.
\end{proposition}
\begin{proof}
We plug the bound on lack of convexity in Lemma~\ref{lem:rho-fhat} in duality gap bound from e.g. \citep[App.I,\,Th.\,3]{Ekel99}.
\end{proof}



\paragraph{Primalization}

Note that not all optimal solutions to the relaxation in~\eqref{eq:lasso-relax} have an objective in~\eqref{eq:lasso-l0} satisfying the bound in~\eqref{eq:bnd-pen}. However, because all the constraints in problem~\eqref{eq:lasso-l0} are linear, we can use the randomized post-processing procedure in~\citep{Udel16} to extract feasible points of~\eqref{eq:lasso-l0} satisfying~\eqref{eq:bnd-pen}. Large-scale algorithms to perform this post-processing step using ADDMM are described in \citep[\S7.1]{Udel16}.



==> general.tex <==
\section{General Case}
\label{sec:general}

Consider the following optimization problem
\begin{align}\label{eq:gen}
    \min_x &\; \sum_i f_i(x_i,z_i)  \\
    &\text{s.t} \;\;\; \|x_i\|_0 \leq k, \; i = 1,\hdots, m \nonumber \\
    & \;\;\;\;\;\; z_i = L_i^\top x_i, \; i = 1,\hdots,m \nonumber
\end{align}
where $x_i, z_i, L_i$ are vectors and matrices of appropriate sizes and $m$ is the number of components for which $f$ has a block decomposable structure. In the sequel we consider $m=1$ and the results trivially extend for general $m$.\\



==> notations.tex <==
%!TEX root = main.tex

% Weird Macros

\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}

% Theorems
%\usepackage[colorlinks,citecolor=blue,urlcolor=black,linkcolor=blue,pdfborder={0 0 0}]{hyperref}

\usepackage[capitalize]{cleveref}  
\crefname{nlem}{Lemma}{Lemmas}
\crefname{nprop}{Proposition}{Propositions}
\crefname{ncor}{Corollary}{Corollaries}
\crefname{nthm}{Theorem}{Theorems}
\crefname{exa}{Example}{Examples}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{equation}{}{}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}{Fact}
\theoremstyle{definition}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}


% Operator

\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\diag}{\text{diag}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\grad}{\nabla}
\newcommand{\hess}{\nabla^2}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\fracpar}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\Ind}[1]{\mathbbm{1}{#1}}

% Math
% some traditional defintions that can be blamed on craig barratt
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}

% arash added these two
\newcommand{\BA}{\begin{array}}
\newcommand{\EA}{\end{array}}

% Refs, etc
\newcommand{\refp}[1]{(\ref{#1})}

% text abbrevs
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}
\newcommand{\ones}{\mathbf 1}
\newcommand{\con}{\text{con}}
\newcommand{\pen}{\text{pen}}

% std math stuff
\newcommand{\reals}{{\mathbb R}}
\newcommand{\sreals}{\scriptsize{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\complex}{{\mbox{\bf C}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

% lin alg stuff
\newcommand{\Span}{\mbox{\textrm{span}}}
\newcommand{\Range}{\mbox{\textrm{range}}}
\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\diam}{\mathop{\bf diam}}
\newcommand{\sphere}{{\mathbb S}}
\newcommand{\Nullspace}{\mbox{\textrm{nullspace}}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\NumRank}{\mathop{\bf NumRank}}
\newcommand{\NumCard}{\mathop{\bf NumCard}}
\newcommand{\Card}{\mathop{\bf Card}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}
%XXX dumb question: do we not use \diag(...) to form diagonal or 
%block diagonal matrices?
\newcommand{\idm}{\mathbf{I}}

% probability stuff
\newcommand{\Expect}{\textstyle\mathop{\bf E}}
\newcommand{\Median}{\textstyle\mathop{\bf M}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\erf}{\mathop{\bf erf}}

% convexity & optimization stuff
\newcommand{\Co}{{\mathop {\bf Co}}}
\newcommand{\co}{{\mathop {\bf Co}}}
\newcommand{\Ext}{{\mathop {\bf Ext}}}
\newcommand{\Var}{\mathop{\bf var{}}}
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\Ltwo}{{\bf L}_2}
\newcommand{\QED}{~~\rule[-1pt]{6pt}{6pt}}\def\qed{\QED}
\newcommand{\approxleq}{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\newcommand{\epi}{\mathop{\bf epi}}
%\newcommand{\hypo}{\mathop{\bf hypo}}
\newcommand{\var}{\mathop{\bf var}}

\newcommand{\vol}{\mathop{\bf vol}}
\newcommand{\Vol}{\mathop{\bf vol}}

\newcommand{\dom}{\mathop{\bf dom}}
\newcommand{\aff}{\mathop{\bf aff}}
\newcommand{\cl}{\mathop{\bf cl}}
\newcommand{\Angle}{\mathop{\bf angle}}
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\relint}{\mathop{\bf rel int}}
\newcommand{\bd}{\mathop{\bf bd}}
\newcommand{\dsp}{\displaystyle}
\newcommand{\foequal}{\simeq}
\newcommand{\VOL}{{\mbox{\bf vol}}}
\newcommand{\xopt}{x^{\rm opt}}

%the following ones seem way too specialized to be here...
%let's omve them to a new file called defs2.tex or something like that
\newcommand{\Xb}{{\mbox{\bf X}}}
\newcommand{\xst}{x^\star}
\newcommand{\varphist}{\varphi^\star}
\newcommand{\lambdast}{\lambda^\star}
\newcommand{\Zst}{Z^\star}
\newcommand{\fstar}{f^\star}
\newcommand{\xstar}{x^\star}
\newcommand{\xc}{x^\star}
\newcommand{\lambdac}{\lambda^\star}
\newcommand{\lambdaopt}{\lambda^{\rm opt}}

% defs for cones & generalized inequalities
\newcommand{\geqK}{\mathrel{\succeq_K}}
\newcommand{\gK}{\mathrel{\succ_K}}
\newcommand{\leqK}{\mathrel{\preceq_K}}
\newcommand{\lK}{\mathrel{\prec_K}}
\newcommand{\geqKst}{\mathrel{\succeq_{K^*}}}
\newcommand{\gKst}{\mathrel{\succ_{K^*}}}
\newcommand{\leqKst}{\mathrel{\preceq_{K^*}}}
\newcommand{\lKst}{\mathrel{\prec_{K^*}}}
\newcommand{\geqL}{\mathrel{\succeq_L}}
\newcommand{\gL}{\mathrel{\succ_L}}
\newcommand{\leqL}{\mathrel{\preceq_L}}
\newcommand{\lL}{\mathrel{\prec_L}}
\newcommand{\geqLst}{\mathrel{\succeq_{L^*}}}
\newcommand{\gLst}{\mathrel{\succ_{L^*}}}
\newcommand{\leqLst}{\mathrel{\preceq_{L^*}}}
\newcommand{\lLst}{\mathrel{\prec_{L^*}}}

% From Alex
\newcommand{\realsp}{\mathbb{R}_+^n}
\newcommand{\intrealsp}{\int_{\mathbf{R}_+^n}}
\newcommand{\rank}{\textbf{rank}}


==> prelim.tex <==
%!TEX root = nonlin.tex
\section{Preliminaries}
\label{sec:prelim}


==> primalization.tex <==
%!TEX root = main.tex
\section{Primalization}
\label{sec:prim}
Recall the \eqref{eq:primal} is equivalent to
\begin{align*}
    p^\ast(k) = \min_{u,z,v} &\;\; \dfrac{1}{2}v^\top \Lambda^{1/2} D_u \Lambda^{1/2} v + \dfrac{1}{2} z^\top z + p^\top D_u v \\
     \text{s.t} &\;\;\;\; L^\top D_u v = z \\
    & \;\;\;\; u \in \{0,1\}^m \\
    & \;\;\;\; \ones^\top u \leq k
\end{align*}
where $D_u = \diag(u_1,\hdots,u_m)$. Consider the relaxed problem
\begin{align*}
    d^\ast(k) = \min_{u,z,v} &\;\; \dfrac{1}{2}v^\top \Lambda^{1/2} D_u \Lambda^{1/2} v + \dfrac{1}{2} z^\top z + p^\top D_u v \\
     \text{s.t} &\;\;\;\; L^\top D_u v = z \\
    & \;\;\;\; u \in [0,1]^m \\
    & \;\;\;\; \ones^\top u \leq k
\end{align*}
where we relax the binary constraint on $u$. \textbf{Note that this is exactly equivalent to the bidual \eqref{eq:BD-QP} since we can invert the analysis in Lemma 1 in which we arrived at \eqref{eq:primal-mm}.} In epigraph form, the problem writes
\begin{align*}
    \min_{t,u,z,v} &\;\; t \\
    \text{s.t} & \;\;\;\; \begin{bmatrix}
    t^\ast \\
    k \\
    0_r
    \end{bmatrix} \in \begin{bmatrix}
    \tfrac{1}{2}\|z\|_2^2 \\
    \mathbb{R}_+ \\
    -z
    \end{bmatrix} + \sum_{i=1}^m u_i \begin{bmatrix}
    \lambda_i v_i^2 + p_i v_i \\
    1 \\
    \ell_i v_i
    \end{bmatrix}
\end{align*}
Now let $u^\ast, v^\ast, z^\ast, t^\ast$ be optimal solutions. This implies
\begin{align*}
    \begin{bmatrix}
    t^\ast \\
    k - s_1 \\
    0_r
    \end{bmatrix} &= \begin{bmatrix}
    \tfrac{1}{2}\|z^\ast\|_2^2 \\
    0 \\
    -z^\ast
    \end{bmatrix} + \sum_{i=1}^m u_i^\ast \begin{bmatrix}
    \lambda_i v_i^{\ast^2} + p_i v_i^\ast \\
    1 \\
    \ell_i v_i^\ast
    \end{bmatrix} \\
    &= \begin{bmatrix}
    \tfrac{1}{2}\|z^\ast\|_2^2 \\
    0 \\
    -z^\ast
    \end{bmatrix} + 
    \sum_{i=1}^m  \Co\left(\left\{0 , \begin{bmatrix}
    \lambda_i v_i^{\ast^2} + p_i v_i^\ast \\
    1 \\
    \ell_i v_i^\ast
    \end{bmatrix} \right\}\right)
\end{align*}
for some $s_1 \geq 0$. Now, the Shapley Folkman theorem \citep{Star69} states that if 
\begin{align*}
    x \in \sum_{i=1}^m  \Co\left(\left\{0 , \begin{bmatrix}
    \lambda_i v_i^{\ast^2} + p_i v_i^\ast \\
    1 \\
    \ell_i v_i^\ast
    \end{bmatrix} \right\}\right)
\end{align*}
then
\begin{align*}
    x \in \sum_{i \in S} \Co\left(\left\{0 , \begin{bmatrix}
    \lambda_i v_i^{\ast^2} + p_i v_i^\ast \\
    1 \\
    \ell_i v_i^\ast
    \end{bmatrix} \right\}\right) + \sum_{i \in S^c} \left(\left\{0 , \begin{bmatrix}
    \lambda_i v_i^{\ast^2} + p_i v_i^\ast \\
    1 \\
    \ell_i v_i^\ast
    \end{bmatrix} \right\}\right)
\end{align*}
where $|S| \leq r + 2$. In particular, there exists $\bar{u}$ such that
\begin{align*}
    x = \sum_{i \in S} \bar{u_i} \begin{bmatrix}
    \lambda_i v_i^{\ast^2} + p_i v_i^\ast \\
    1 \\
    \ell_i v_i^\ast
    \end{bmatrix} + \sum_{i \in S^c} \bar{u}_i\begin{bmatrix}
    \lambda_i v_i^{\ast^2} + p_i v_i^\ast \\
    1 \\
    \ell_i v_i^\ast
    \end{bmatrix}
\end{align*}
where $S = \{i : \bar{u}_i \not \in \{0,1\}\}$. \\

Suppose we can compute this $\bar{u}$ (i.e. via linear programming). Now define
\begin{align*}
    \begin{cases}
    \tilde{u}_i = \bar{u}_i, \;\tilde{v}_i = v_i^\ast & \text{if $i \not \in S$} \\
    \tilde{u}_i = 1, \;\tilde{v}_i = \bar{u}_i v_i^\ast  & \text{if $i \in S$}
    \end{cases}
\end{align*}
We claim that $(\tilde{u}, \tilde{v})$ (and the resulting $\tilde{z}$ and $\tilde{t}$) are feasible for the problem defining $p^\ast(k+r+2)$ and $p^\ast(k+r+2) \leq d^\ast(k) \leq p^\ast(k)$. It is clear that $d^\ast(k) \leq p^\ast(k)$. All that remains to show is that $(\tilde{u}, \tilde{v}, \tilde{z}, \tilde{t})$ is feasible for the problem defining $p^\ast(k+r+2)$ and that the objective value of $(\tilde{u}, \tilde{v}, \tilde{z}, \tilde{u})$ is less than that of $(\bar{u}, v^\ast, z^\ast, t^\ast)$. Since the solutions agree on $S^c$ we only need to compare the objective value on $S$. For $i \in S$, note that the objectives are
\begin{align*}
    \tfrac{1}{2} \lambda_i \bar{u_i}^\ast v_i^{\ast^2} + p_i \bar{u}_i v_i^\ast
\end{align*}
and 
\begin{align*}
    \tfrac{1}{2} \lambda_i \tilde{u}_i \tilde{v}_i^2 + p_i \tilde{u}_i \tilde{v}_i = \tfrac{1}{2} \lambda_i \bar{u}_i^2 v_i^{\ast^2} + p_i \bar{u}_i v_i^\ast
\end{align*}
Note furthermore that $\tilde{z} = z^\ast$ since
\begin{align*}
    z^\ast &= \sum_{i \in S} \ell_i \bar{u}_i v_i^\ast + \sum_{i \not \in S} \ell_i \bar{u}_i v_i^\ast \\
    &= \sum_{i \in S} \ell_i \tilde{u_i} \tilde{v_i} + + \sum_{i \not \in S} \ell_i \bar{u}_i v_i^\ast \\
    &= \tilde{z}
\end{align*}
As a result $\|z^\ast\|_2^2 = \|\tilde{z}\|_2^2$ and indeed the objective value of $(\tilde{u}, \tilde{v}, \tilde{z}, \tilde{t})$ is less than that of $(u^\ast, v^\ast, z^\ast, t^\ast)$ concluding the proof.
% \textbf{I think this analysis requires that support set S is the same as optimal $u^\ast$}


==> primalization_clean.tex <==
%!TEX root = main.tex
\section{Primalization}
\label{sec:prim}
Recall \eqref{eq:primal-mm}
\begin{align*}
    p^\ast(k) = \min_{\substack{v \in \mathbb{R}^r, u \in \{0,1\}^m \\ \ones^\top u \leq k}} \dfrac{1}{2}v^\top (I_r + L^\top \Sigma_u L ) v - v^\top L^\top \Sigma_u p
\end{align*}
where $\Sigma_u = \Lambda^{1/2} \diag(u_1,\hdots,u_m) \Lambda^{1/2}$ and the bidual
\begin{align*}
    p^{\ast \ast}(k) &= \min_{\substack{v \in \mathbb{R}^r, u \in [0,1]^m \\ \ones^\top u \leq k}} \dfrac{1}{2}v^\top (I_r + L^\top \Sigma_u L ) v - v^\top L^\top \Sigma_u p \\
    &= \min_{\substack{v \in \mathbb{R}^r, u \in [0,1]^m \\ \ones^\top u \leq k}} \dfrac{1}{2} \|v\|_2^2 + \dfrac{1}{2}\sum_{i=1}^m \; u_i \lambda_i (\ell_i^\top v)\Big[ \ell_i^\top v - p_i \Big] 
\end{align*}
where we relax the binary constraint on $u$. In epigraph form, the problem writes
\begin{align*}
    \min_{t,u,z,v} &\;\; t \\
    \text{s.t} & \;\;\;\; \begin{bmatrix}
    t^\ast \\
    k 
    \end{bmatrix} \in \begin{bmatrix}
    0 \\
    \mathbb{R}_+ 
    \end{bmatrix} + \sum_{i=1}^m u_i \begin{bmatrix}
    (1+\lambda_i) (\ell_i^\top v)^2 - \lambda_i p_i (\ell_i^\top v) \\
    1 
    \end{bmatrix}
\end{align*}
Now let $u^\ast, v^\ast, t^\ast$ be optimal solutions. This implies
\begin{align*}
    \begin{bmatrix}
    t^\ast \\
    k - s_1 
    \end{bmatrix} &=  \sum_{i=1}^m u_i^\ast \begin{bmatrix}
    (1+\lambda_i) (\ell_i^\top v^\ast)^2 - \lambda_i p_i (\ell_i^\top v^\ast) \\
    1 
    \end{bmatrix} \\
    &= \sum_{i=1}^m  \Co\left(\left\{0 , \begin{bmatrix}
    (1+\lambda_i) (\ell_i^\top v^\ast)^2 - \lambda_i p_i (\ell_i^\top v^\ast) \\
    1 
    \end{bmatrix}  \right\}\right)
\end{align*}
for some $s_1 \geq 0$. Now, the Shapley Folkman theorem \citep{Star69} states that if 
\begin{align*}
    x \in \sum_{i=1}^m  \Co\left(\left\{0 , \begin{bmatrix}
    (1+\lambda_i) (\ell_i^\top v^\ast)^2 - \lambda_i p_i (\ell_i^\top v^\ast) \\
    1 
    \end{bmatrix}  \right\}\right)
\end{align*}
then
\begin{align*}
    x \in \sum_{i \in S} \Co\left(\left\{0 , \begin{bmatrix}
    (1+\lambda_i) (\ell_i^\top v^\ast)^2 - \lambda_i p_i (\ell_i^\top v^\ast) \\
    1 
    \end{bmatrix}  \right\}\right) + \sum_{i \in S^c} \left(\left\{0 , \begin{bmatrix}
    (1+\lambda_i) (\ell_i^\top v^\ast)^2 - \lambda_i p_i (\ell_i^\top v^\ast) \\
    1 
    \end{bmatrix}  \right\}\right)
\end{align*}
where $|S| \leq 2$. In particular, there exists $\bar{u}$ such that
\begin{align*}
    x = \sum_{i \in S} \bar{u_i} \begin{bmatrix}
    (1+\lambda_i) (\ell_i^\top v^\ast)^2 - \lambda_i p_i (\ell_i^\top v^\ast) \\
    1 
    \end{bmatrix}  + \sum_{i \in S^c} \bar{u}_i\begin{bmatrix}
    (1+\lambda_i) (\ell_i^\top v^\ast)^2 - \lambda_i p_i (\ell_i^\top v^\ast) \\
    1 
    \end{bmatrix} 
\end{align*}
where $S = \{i : \bar{u}_i \not \in \{0,1\}\}$. \\

Suppose we can compute this $\bar{u}$ (i.e. via linear programming). Now define
\begin{align*}
    \begin{cases}
    \tilde{u}_i = \bar{u}_i, \;\tilde{v}_i = v_i^\ast & \text{if $i \not \in S$} \\
    \tilde{u}_i = 1, \;\tilde{v}_i = \bar{u}_i v_i^\ast  & \text{if $i \in S$}
    \end{cases}
\end{align*}
We claim that $(\tilde{u}, \tilde{v})$ (and the resulting $\tilde{z}$ and $\tilde{t}$) are feasible for the problem defining $p^\ast(k+r+2)$ and $p^\ast(k+r+2) \leq d^\ast(k) \leq p^\ast(k)$. It is clear that $d^\ast(k) \leq p^\ast(k)$. All that remains to show is that $(\tilde{u}, \tilde{v}, \tilde{z}, \tilde{t})$ is feasible for the problem defining $p^\ast(k+r+2)$ and that the objective value of $(\tilde{u}, \tilde{v}, \tilde{z}, \tilde{u})$ is less than that of $(\bar{u}, v^\ast, z^\ast, t^\ast)$. Since the solutions agree on $S^c$ we only need to compare the objective value on $S$. For $i \in S$, note that the objectives are
\begin{align*}
    \tfrac{1}{2} \lambda_i \bar{u_i}^\ast v_i^{\ast^2} + p_i \bar{u}_i v_i^\ast
\end{align*}
and 
\begin{align*}
    \tfrac{1}{2} \lambda_i \tilde{u}_i \tilde{v}_i^2 + p_i \tilde{u}_i \tilde{v}_i = \tfrac{1}{2} \lambda_i \bar{u}_i^2 v_i^{\ast^2} + p_i \bar{u}_i v_i^\ast
\end{align*}
Note furthermore that $\tilde{z} = z^\ast$ since
\begin{align*}
    z^\ast &= \sum_{i \in S} \ell_i \bar{u}_i v_i^\ast + \sum_{i \not \in S} \ell_i \bar{u}_i v_i^\ast \\
    &= \sum_{i \in S} \ell_i \tilde{u_i} \tilde{v_i} + + \sum_{i \not \in S} \ell_i \bar{u}_i v_i^\ast \\
    &= \tilde{z}
\end{align*}
As a result $\|z^\ast\|_2^2 = \|\tilde{z}\|_2^2$ and indeed the objective value of $(\tilde{u}, \tilde{v}, \tilde{z}, \tilde{t})$ is less than that of $(u^\ast, v^\ast, z^\ast, t^\ast)$ concluding the proof.
% \textbf{I think this analysis requires that support set S is the same as optimal $u^\ast$}


==> sdp.tex <==
\section{Rank Constrained SDP}
\label{sec:sdp}

Consider the following SDP
\begin{align*}
    \min_{X \succeq 0, \; \rank (X) \leq k} \; f(X) + \dfrac{\gamma}{2}\|X\|_F^2
\end{align*}

This problem is equivalent to 
\begin{align*}
    \min_{V, u \in \{0,1\}^m} \; f(VD_u V^\top) + \dfrac{\gamma}{2}\|V D_u V^\top\|_F^2 \; : \; \ones^\top u \leq k
\end{align*}
via a spectral decomposition of $X = V D_u V^\top = V \diag(u_1,\hdots, u_m) V^\top$ where $V^\top V = S$ is diagonal. Rewriting $f(\cdot)$ using its fenchel conjugate, we have via weak duality
\begin{align}
    \max_{Z} -f^\ast (Z) + \min_{V, u \in \{0,1\}^m} \langle Z, VD_uV^\top \rangle + \dfrac{\gamma}{2} \|VD_u V^\top\|_F^2 \; : \; \ones^\top u \leq k
\end{align}
The hope is that minimizing over $V$ (in closed form) results in a function that is linear in $u$. The rest of the analysis done before will follow exactly then.
